Marco DeepResearch: Unlocking Efficient Deep Research Agents via Verification-Centric Design

Deep research agents autonomously conduct open-ended investigations, integrating complex information retrieval with multi-step reasoning across diverse sources to solve real-world problems. To sustain this capability on long-horizon tasks, reliable verification is critical during both training and inference. A major bottleneck in existing paradigms stems from the lack of explicit verification mechanisms in QA data synthesis, trajectory construction, and test-time scaling. Errors introduced at each stage propagate downstream and degrade the overall agent performance. To address this, we present Marco DeepResearch, a deep research agent optimized with a verification-centric framework design at three levels: \textbf{(1)~QA Data Synthesis:} We introduce verification mechanisms to graph-based and agent-based QA synthesis to control question difficulty while ensuring answers are unique and correct; \textbf{(2)~Trajectory Construction:} We design a verification-driven trajectory synthesis method that injects explicit verification patterns into training trajectories; and \textbf{(3)~Test-time scaling:} We use Marco DeepResearch itself as a verifier at inference time and effectively improve performance on challenging questions. Extensive experimental results demonstrate that our proposed Marco DeepResearch agent significantly outperforms 8B-scale deep research agents on most challenging benchmarks, such as BrowseComp and BrowseComp-ZH. Crucially, under a maximum budget of 600 tool calls, Marco DeepResearch even surpasses or approaches several 30B-scale agents, like Tongyi DeepResearch-30B.

==> Marco_DeepResearch/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Marco_DeepResearch/sections/abstract.tex <==
% =============================================================================
% Abstract
% =============================================================================
% NOTE: The abstract is now defined in main.tex (before \begin{document})
% as required by the paper_improved.cls template.
% This file is kept for reference only.
% =============================================================================


==> Marco_DeepResearch/sections/conclusion.tex <==
% =============================================================================
% Section 9: Conclusion
% =============================================================================

\section{Conclusion}
\label{sec:conclusion}

This paper addresses a bottleneck in current deep research agents: the lack of explicit verification across QA data synthesis, trajectory construction, and inference, which leads to error propagation and under-utilized test-time computation. To solve this, we propose Marco DeepResearch, a 8B-scale deep search agent that optimized by our proposed verification-centric design with three improvements: verified QA synthesis, verification-driven trajectory construction, and verifier-guided test-time scaling. Extensive experimental results demonstrate that our proposed Marco DeepResearch agent significantly outperforms 8B-scale open-source deep search agents on most benchmarks BrowseComp and BrowseComp-ZH, and surpasses several 30B-scale deep search agents on BrowseComp-ZH. Furthermore, detailed analysis and ablation study verify the positive contributions of our verification-centric designs.


==> Marco_DeepResearch/sections/data_synthesis.tex <==
% =============================================================================
% Section 3: Enhanced Data Synthesis (QA Data Synthesis)
% =============================================================================

\section{Enhanced Data Synthesis}
\label{sec:data-synthesis}

High-quality question--answer (QA) data forms the foundation for training deep research agents.
In this section, we present our enhanced data synthesis pipeline, which addresses the limitations of existing approaches in terms of quality, realism, difficulty, and diversity.

\subsection{Problem Analysis}
\label{sec:data-problem}

We identify three primary limitations of current QA data synthesis methods for deep research agent training:

\paragraph{Insufficient realism.}
Knowledge-graph-based synthesis methods~\cite{KG-QA-synthesis-refs} construct questions by composing entities and relations from structured knowledge bases.
% cite: knowledge-graph-based QA synthesis papers
While this produces questions with verifiable answers, the resulting queries often fail to reflect real-world information-seeking scenarios.
Questions derived from static knowledge graphs (e.g., those built from Wikipedia) are frequently anchored to a fixed temporal snapshot and may be trivially resolvable through alternative web sources, undermining their value as training signals for agents that must operate in dynamic, open-ended web environments.

\paragraph{Unreliable quality.}
Approaches that synthesize questions through real web exploration~\cite{SAGE} improve authenticity but introduce quality concerns.
% cite: SAGE
Without rigorous verification, synthesized answers may contain hallucinations, be non-unique across different web sources, or fail to meet the expected level of specificity and factual precision.
The open-ended nature of web information makes automated quality control inherently challenging, leading to noisy training signals that can degrade model performance.

\paragraph{Limited diversity.}
Most existing pipelines employ a single synthesis strategy, which inherently limits the diversity of the resulting dataset along multiple dimensions: problem type (factual retrieval vs.\ multi-step reasoning vs.\ analytical comparison), difficulty level (simple lookups vs.\ complex multi-hop chains), domain coverage (science, history, finance, etc.), and required reasoning patterns.
This lack of diversity constrains the model's ability to generalize across the broad spectrum of research scenarios encountered in practice.


\subsection{Knowledge-Graph-Augmented Real Web Exploration}
\label{sec:data-graph-web}

To simultaneously address realism and difficulty, we combine knowledge graph construction with real web exploration.
Our approach draws inspiration from existing graph-based and web-based methods~\cite{Step-DeepResearch, MiroThinker} while introducing key enhancements.
% cite: Step-DeepResearch (real web grounding), MiroThinker (MultiDocQA synthesis)

\paragraph{Graph construction with web grounding.}
We begin by constructing knowledge graphs from diverse, high-quality sources including encyclopedias, academic repositories, and curated web collections.
For each entity node in the graph, we perform real web exploration to identify and associate relevant web pages, grounding the abstract graph structure in authentic, accessible web content.
This web-grounding step serves two purposes: it ensures that the resulting questions require genuine web-based information seeking to resolve, and it anchors the questions in the current state of the web rather than a static knowledge snapshot.

\paragraph{Difficulty control.}
We implement explicit difficulty control mechanisms to produce questions spanning a range of complexity levels.
Specifically, we vary the number of reasoning hops required, the degree of constraint obfuscation applied to entity references, and the diversity of source domains that must be integrated.
\textcolor{red}{[To be elaborated with specific difficulty control parameters and examples.]}

\paragraph{Timeliness and authenticity.}
By associating graph nodes with real web pages and validating question answerability against live web content, our pipeline ensures that synthesized questions reflect current web conditions.
This addresses a key weakness of purely graph-based methods, where temporal drift between graph construction and model deployment can render questions unrealistic.



\subsection{Three-Agent QA Verification Framework}
\label{sec:data-verification}

To ensure the quality and factual reliability of synthesized QA pairs, we introduce a dedicated three-agent verification framework.
Unlike single-pass generation approaches, our framework employs specialized agents that independently validate different aspects of data quality.

\paragraph{Question agent.}
The question agent is responsible for generating complex, multi-hop questions by exploring real web environments and synthesizing information across multiple sources.
It produces candidate questions along with preliminary answers derived from the explored web content.
The question agent is instructed to generate questions that require genuine multi-step reasoning and cannot be resolved through simple keyword matching or single-source retrieval.

\paragraph{Search agent.}
The search agent independently attempts to solve each generated question using the available tool suite (web search, page visits, etc.).
This independent solution attempt serves as a validation mechanism: if the search agent can reliably arrive at the same answer through an independent search process, the question--answer pair is more likely to be well-formed and unambiguous.
The search agent's trajectory also provides valuable signal about the difficulty and solvability of the question.

\paragraph{Verifier agent.}
The verifier agent performs rigorous quality control by independently examining both the question and the candidate answers.
Its verification encompasses multiple dimensions:
\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textbf{Answer correctness:} The verifier cross-checks the proposed answer against independently retrieved evidence, ensuring factual accuracy.
    \item \textbf{Hallucination detection:} The verifier identifies cases where the proposed answer cannot be substantiated by available web evidence, flagging potential hallucinations.
    \item \textbf{Answer uniqueness:} The verifier checks whether alternative valid answers exist, filtering out questions with ambiguous or non-unique solutions.
    \item \textbf{Quality gate:} Questions that fail any verification criterion are either revised (with feedback from the verifier guiding the revision) or discarded, ensuring that only high-quality QA pairs enter the training set.
\end{itemize}

This three-agent verification framework provides controllable quality assurance that is difficult to achieve through single-model generation, as each agent brings an independent perspective that helps identify and eliminate different categories of errors.


\subsection{Diverse Data Synthesis Strategies}
\label{sec:data-diversity}

We argue that data diversity is as important as data quality for training robust deep research agents.
Rather than relying on a single synthesis method, we employ multiple complementary strategies, each contributing unique characteristics to the overall training set.

\paragraph{Multiple synthesis approaches.}
Our data synthesis pipeline incorporates several complementary strategies:
\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textbf{Knowledge-graph-based synthesis:} Produces structured multi-hop questions with well-defined reasoning chains, particularly effective for questions requiring integration of facts across multiple entities and relations.
    \item \textbf{Real web exploration-based synthesis:} Generates questions grounded in authentic web content, capturing the characteristics of real-world information-seeking tasks including temporal sensitivity and source diversity.
    \item \textbf{Sub-task decomposition-based synthesis:} Creates complex questions by composing multiple simpler sub-tasks, each requiring different types of information retrieval or reasoning, resulting in questions that demand structured problem-solving approaches.
    \item \textbf{Hybrid strategies:} Combines elements from the above approaches to produce questions that exhibit characteristics of multiple categories simultaneously.
\end{itemize}

\paragraph{Diversity along multiple dimensions.}
By combining these strategies, our synthesized dataset achieves diversity along four key dimensions:
(1) \textit{problem type diversity}---spanning factual retrieval, multi-step reasoning, comparative analysis, and temporal queries;
(2) \textit{difficulty gradient diversity}---ranging from straightforward lookups to complex chains requiring deep exploration;
(3) \textit{domain coverage diversity}---encompassing science, technology, history, finance, law, culture, and other areas;
and (4) \textit{trajectory pattern diversity}---reflecting different search strategies, reasoning paths, and interaction depths.

\paragraph{Empirical evidence for complementarity.}
\textcolor{red}{[To be filled with experimental evidence showing that each synthesis strategy contributes additive performance gains, and that the combined dataset outperforms any single-strategy dataset. This will be cross-referenced with the analysis experiments in Section~\ref{sec:experiments}.]}


==> Marco_DeepResearch/sections/experiments.tex <==
% =============================================================================
% Section 7: Experiments
% =============================================================================

\section{Experimental Setup}
\label{sec:exp-setup}

\paragraph{Benchmarks.}
We evaluate our proposed Marco DeepResearch agent on six deep search benchmarks: (1) \textbf{BrowseComp}~\cite{wei2025browsecompsimplechallengingbenchmark}:
Measuring agent's information seeking capability by navigating the web; (2) \textbf{BrowseComp-ZH}~\cite{zhou2025browsecompzhbenchmarkingwebbrowsing}: Chinese counterpart evaluating agentic information seeking; (3) \textbf{GAIA (text-only)}~\cite{mialon2023gaiabenchmarkgeneralai}: Real-world multi-step questions for general AI assistants; (4) \textbf{xBench-DeepSearch}~\cite{xBench-DeepSearch}: Deep search across diverse domains\footnote{Both 2505 and 2510 splits are evaluated.}; (5) \textbf{WebWalkerQA}~\cite{wu2025webwalkerbenchmarkingllmsweb}: Multi-step web navigation and information extraction; and (6) \textbf{DeepSearchQA}~\cite{gupta2026deepsearchqabridgingcomprehensivenessgap}: Evaluating exhaustive answer set generation through multi-source retrieval, entity resolution, and stopping criteria reasoning.

\paragraph{Baselines.}
We compare against three groups of state-of-the-art baselines: (1) \textbf{Foundation models with tools}: GLM-4.7~\cite{5team2026glm5vibecodingagentic}, Minimax-M2.1, DeepSeek-V3.2~\cite{deepseekai2025deepseekv32pushingfrontieropen}, Kimi-K2.5~\cite{kimiteam2026kimik25visualagentic}, Claude-Sonnet/Opus, OpenAI-o3, GPT-5 High and Gemini-3-Pro;  (2) \textbf{Trained agents $\geq$ 30B-scale}: Tongyi DeepResearch~\cite{team2025tongyi}, WebSailor-v2~\cite{li2025websailornavigatingsuperhumanreasoning}, MiroThinker-v1.0/v1.5/v1.7~\cite{miromind2025mirothinker,miromindteam2026mirothinker17h1heavyduty}, DeepMiner~\cite{tang2025turnlimitstrainingdeep}, OpenSeeker-30B-SFT~\cite{du2026openseekerdemocratizingfrontiersearch}, and SMTL~\cite{chen2026searchmorethinkless}; and (3) \textbf{Trained agents $\leq$ 8B-scale}: MiroThinker-v1.0-8B, WebExplorer-8B-RL~\cite{liu2025webexplorerexploreevolvetraining}, AgentCPM-Explore-4B~\cite{AgentCPMExplore2026} and RE-TRAC-4B~\cite{zhu2026retracrecursivetrajectorycompression}.

\paragraph{Training Data.}
Our training corpus contains two sources: \textbf{(1) Open-source data}, including 2WikiMultihopQA~\cite{ho2020constructingmultihopqadataset}, BeerQA~\cite{qi2021answeringopendomainquestionsvarying}, ASearcher~\cite{gao2025turnsunlockinglonghorizonagentic}, DeepDive~\cite{lu2025deepdiveadvancingdeepsearch}, QA-Expert-Multi-Hop-QA~\cite{qa-expert}, and REDSearcher~\cite{chu2026redsearcherscalablecostefficientframework}; and \textbf{(2) Synthetic data}, including (i) real-world e-commerce business-development datasets from our inner applications~\cite{lan2025deepwidesearchbenchmarkingdepthwidth,yang2025hscodecomprealisticexpertlevelbenchmark,lan2026tableassearchformulatelonghorizonagentic} and (ii) data synthesized by our verified data synthes. In details, we collect over 12K synthesized graph-based QA and agent-based QA samples. Moreover, we hold-out over 2K high-quality QA samples for RL training. Trajectory data are synthesized using frontier foundation models, including Qwen3.5-Plus, GLM-5, and Kimi-K2, among others, followed by data cleaning (e.g., tool-call error correction).

\paragraph{Implementation Details.}
%\paragraph{Training details.}
We use Qwen3-8B as the backbone. YaRN is used to extend the context window to 128K. Supervised fine-tuning and RL are conducted on 64 A100 GPUs using Megatron~\cite{megatron-lm}. 
%Reinforcement learning runs on the same 64 A100 GPUs with FSDP2 (SP=4, TP=2, PP=2), batch size 128, 16 rollout samples per query.
To improve system efficiency and stability, we use Redis-based caching for repeated queries/pages, exponential-backoff retries for transient failures, asynchronous non-blocking tool calls, asynchronous reward computation pipelined with model updates, and synchronized deployment of the WebVisit summary model as an independent training-cluster service~\cite{AgentCPMExplore2026}.
%\paragraph{Evaluation details.}
As for the evaluation details, we follow previous works~\cite{miromind2025mirothinker} and evaluate Marco DeepResearch agent under a maximum budget of 600 tool calls. Decoding uses temperature $0.7$, top-$p$ $0.95$, and a maximum generation length of 16{,}384 tokens.

\section{Experimental Results}
\subsection{Main Results}
\label{sec:exp-main}
\begin{table}[t]
\centering
\caption{Performance on deep search benchmarks. Best open-source results are \textbf{bolded} and the second-best are \underline{underlined}. Results marked with $^\star$ are evaluated using our implementation.}
\label{tab:main-results}
\small
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c}
\toprule
%\textbf{Model} & \textbf{BrowseComp} & \textbf{BrowseComp-ZH} & \textbf{GAIA} & \textbf{WebWakerQA} & \textbf{xBench-DS-2505} \\
\textbf{Model} & \begin{tabular}{@{}c@{}}\textbf{Browse} \\ \textbf{Comp}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Brows} \\ \textbf{Comp-ZH}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{GAIA} \\ \textbf{text-only}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Web} \\ \textbf{WalkerQA}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{xBench-} \\ \textbf{DS-2505}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{xBench-} \\ \textbf{DS-2510}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Deep} \\ \textbf{SearchQA}\end{tabular} \\
\midrule
\multicolumn{6}{l}{\textbf{Foundation Models with Tools}} \\
\midrule
GLM-4.7 & 67.5 & 66.6 & 61.9 & -- & 72.0 & 52.3 & -- \\
Minimax-M2.1 & 62.0 & 47.8 & 64.3 & -- & 68.7 & 43.0 & --\\
DeepSeek-V3.2 & 67.6 & 65.0 & 75.1 & -- & 78.0 & 55.7 & 60.9 \\
%Kimi-K2-0905 & 7.4 & 22.2 & 60.2 & -- & 61.0 \\
Kimi-K2.5 & 74.9 & 62.3 & -- & -- & -- & 46.0 & 77.1 \\
Claude-4-Sonnet & 12.2 & 29.1 & 68.3 & 61.7 & 64.6 & -- & -- \\
Claude-4.5-Opus & 67.8 & 62.4 & -- & -- & -- & -- & 80.0 \\
OpenAI-o3 & 49.7 & 58.1 & -- & 71.7 & 67.0 & -- & -- \\
OpenAI GPT-5 High & 54.9 & 65.0 & 76.4 & -- & 77.8 & 75.0 & 79.0 \\
Gemini-3.0-Pro & 59.2 & 66.8 & -- & -- & -- & 53.0 & 76.9 \\
\midrule
\multicolumn{6}{l}{\textbf{Trained Agents ($\geq$30B)}} \\
\midrule
MiroThinker-v1.7-mini & 67.9 & 72.3 & 80.3 & -- & -- & 57.2 & 67.9 \\
MiroThinker-v1.5-235B & 69.8 & 71.5 & 80.8 & -- & 77.1 & -- & --\\
MiroThinker-v1.5-30B & 56.1 & 66.8 & 72.0 & -- & 73.1& -- & --\\
MiroThinker-v1.0-72B & 47.1 & 55.6 & 81.9 & 62.1 & 77.8 & -- & -- \\
MiroThinker-v1.0-30B & 41.2 & 47.8 & 73.5 & 61.0 & 70.6 & -- & -- \\
SMTL-30B-300 & 48.6 & -- & 75.7 & 76.5 & 82.0 & -- & --\\
Tongyi-DR-30B & 43.4 & 46.7 & 70.9 & 72.2 & 75.0 & 55.0 & --\\
WebSailor-V2-30B & 35.3 & 44.1 & 74.1 & -- & 73.7& -- & -- \\
DeepMiner-32B-RL & 33.5 & 40.1 & 58.7 & -- & 62.0 & -- & --\\
OpenSeeker-30B-SFT & 29.5 & 48.4 & -- & -- & 74.0 & -- & --\\
\midrule
\multicolumn{6}{l}{\textbf{Trained Agents ($\leq$8B)}} \\
\midrule
AgentCPM-Explore-4B & 24.1 & 29.1 & 63.9 & \underline{68.1} & \underline{70.0} & \underline{34.0}$^{\star}$ & \underline{32.8}$^{\star}$\\
WebExplorer-8B-RL & 15.7 & 32.0 & 50.0 & 62.7 & 53.7 & 23.0$^{\star}$ & 17.8$^{\star}$\\
RE-TRAC-4B & 30.0 & 36.1 & \textbf{70.4} & -- & 74.0 & -- & --\\
MiroThinker-v1.0-8B & \underline{31.1} & \underline{40.2} & 66.4 & 60.6 & 60.6 & \underline{34.0}$^{\star}$ & \textbf{36.7}$^{\star}$ \\
%\multicolumn{6}{l}{\textbf{Marco-DeepResearch-8B (Ours)}} \\
%\textbf{Marco-DR-8B + SFT} & 16.5 & 27.1 & 59.2 & -- & 68.3 & -- & -- \\
%\textbf{Marco-DR-8B + RL} & 17.3 & 29.3 & 61.2 & -- & 75.0 & -- & -- \\
\rowcolor{blue!10} \textbf{Marco-DR-8B (Ours)} & \textbf{31.4} & \textbf{47.1} & \underline{69.9} & \textbf{69.6} & \textbf{82.0} & \textbf{42.0} & 29.2 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

Table \ref{tab:main-results} demonstrates that Marco-DeepResearch-8B outperforms other 8B-scale open-source deep search trained agents on most of benchmarks. 
Specifically, it attains the highest scores in its size category on exploration-heavy tasks, including BrowseComp (31.4), BrowseComp-ZH (47.1), WebWalkerQA (69.6), and xBench-DeepSearch (82.0 on the 2505 split and 42.0 on the 2510 split). For the remaining three benchmarks, our proposed Marco-DeepResearch agent remains highly competitive, missing the top score on GAIA text-only by a marginal 0.5 points compared to RE-TRAC-4B.
Notably, Marco-DeepResearch-8B approaches and even surpasses several competitive 30B-scale deep search agents on several benchmark, like Tongyi-DeepResearch. These results validate the efficacy of our proposed QA data synthesis, trajectory construction methods and test-time scaling strategy, proving that our optimized 8B model can effectively close the performance gap with massive foundation models in complex web navigation and information-seeking tasks.


\subsection{Analysis}
\label{sec:exp-analysis}

We conduct detailed analysis from five aspects: (1) data statistics analysis; (2) effect of QA data verification; (3) ablation study on verification-driven trajectory construction; (4) improvement of reinforcement learning; (5) ablation study on verifier-guided test-time scaling; and (6) context window extension during training.

\paragraph{Data statistics analysis.}

To analyze the strength of our constructed training dataset, we compare our synthesized data with three representative deep search datasets (REDSearcher~\cite{chu2026redsearcherscalablecostefficientframework}, DeepDive~\cite{lu2025deepdiveadvancingdeepsearch} and ASearcher~\cite{gao2025turnsunlockinglonghorizonagentic}) from two perspectives\footnote{The expert trajectory data corresponding to these QA datasets are all constructed using the same agent.}: token length and tool-use depth. Figure~\ref{fig:data-stats-length-tools-open-source} and Figure~\ref{fig:data-stats-length-tools} show that our synthesized samples have both longer token sequences and more tool-call rounds than existing multi-hop and deep search open-source dataset. This shift is important for deep-search training: longer trajectories provide denser supervision on cross-step reasoning, and deeper tool interaction exposes the model to more realistic long-horizon decision patterns. As a result, the model can better learn to maintain state, revise intermediate hypotheses, and complete complex tasks that require extended evidence aggregation.

\begin{figure}[h]
    \centering
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/our_vs_open_token.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/our_vs_open_tool_rounds_optim_clip_50.pdf}
    \end{minipage}
    \caption{Distribution comparison between the open-source multi-hop QA dataset (2Wiki, BeerQA, etc.) and our synthesized data. Left: token count per sample. Right: tool-call rounds per sample.}
    \label{fig:data-stats-length-tools-open-source}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/our_vs_3dataset_token.pdf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/our_vs_3dataset_tool_rounds_optim_clip_50.pdf}
    \end{minipage}
    \caption{Distribution comparison between three deep search data (ASearcher, DeepDive, and REDSearcher) and our synthesized data. Left: token count per sample. Right: tool-call rounds per sample. Our data is consistently shifted toward longer outputs and more tool interactions.}
    \label{fig:data-stats-length-tools}
\end{figure}

Moreover, Figure~\ref{fig:judge-compare} further supports the difficulty of our data. Under the same ReAct-style trajectory construction methods using the same frontier agent, our generated data shows a lower answerable rate than open-source data (29.0\% < 51.7\%), which indicates a harder distribution.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/judge_compare.pdf}
    \caption{Relative to open-source data, our synthesized datasets indicate higher intrinsic difficulty.}
    \label{fig:judge-compare}
\end{figure}



% ==========================================================================
% Ablation 1: Data-Level
% ==========================================================================
%\paragraph{Ablation study on Data Synthesis Methods.}
%We evaluate the contribution of each data source by removing it from the SFT training set while keeping all other components unchanged.
%Table~\ref{tab:data-ablation} shows the contribution of each data component.
%\textcolor{red}{[Results discussion to be written once numbers are available. Expected points:
%(1)~Removing graph-based QA data reduces performance on X, demonstrating the value of knowledge-graph-grounded multi-hop questions with verified answer uniqueness (Section~\ref{sec:qa-graph}).
%(2)~Removing agent-based QA data reduces performance on Y, confirming that realistic web-grounded questions complement graph-based ones (Section~\ref{sec:qa-agent}).
%(3)~Removing trajectory re-rollout data reduces performance, showing that recovered trajectories with reflection behavior patterns contribute to the model's self-correction ability (Section~\ref{sec:trajectory-recovery}).]}
%\begin{table}[h]
%    \centering
%    \caption{Ablation study on data synthesis methods. BC-200-sample indicates the sub-set of BrowseComp with 200 samples.}
%    \label{tab:data-ablation}
%    \small
%    \begin{tabular}{l c c c c}
%    \toprule
%    \textbf{Configuration} & \textbf{BC-200-sample} & \textbf{BC-ZH} & \textbf{GAIA} & \textbf{xBench-DS-2505} \\
%    \midrule
%    Full data (ours) & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}{TBD} \\
%    \quad $-$ Graph-based QA & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}{TBD} \\
%    \quad $-$ Agent-based QA & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}{TBD} \\
    %\quad $-$ Trajectory re-rollout & \textcolor{red}{TBD} & \textcolor{red}{TBD} & \textcolor{red}%{TBD} & \textcolor{red}{TBD} \\
%    \bottomrule
%    \end{tabular}
%\end{table}

\paragraph{Effect of QA data verification.}
To isolate the impact of our adversarial uniqueness verification on data quality, we compare two graph-based synthesis pipelines under identical data scales: one with verification and a baseline without.\footnote{We conduct this ablation using the graph-based approach due to its lower computational overhead. In contrast, agent-based synthesis requires multi-turn web exploration, making data construction prohibitively expensive.} As shown in Table \ref{tab:qa-verification}, integrating this verification step improves downstream performance across most benchmarks. By filtering out noisy and ambiguous samples, verification yields cleaner and more reliable data for subsequent trajectory construction and training.

\begin{table}[h]
    \centering
    \caption{Effect of adversarial uniqueness verification on graph-based QA data quality. Both rows use the same number of QA samples; the difference is whether verification is applied during synthesis. BC-200-sample is a sub-set of BrowseComp with 200 random samples.}
    \label{tab:qa-verification}
    \small
    \begin{tabular}{l c c c c}
    \toprule
    \textbf{QA Synthesis Method} & \textbf{BC-200-sample} & \textbf{BC-ZH} & \textbf{GAIA} & \textbf{xBench-DS-2505} \\
    \midrule
    Graph-based QA (w/o verification) & 14.2 & 24.5 & 55.3 & 67.0 \\
    Graph-based QA (w/ verification)  & 13.8 & 26.8 & 57.6 & 68.3 \\
    \quad \textcolor{red}{$\Delta$ Improvement} & \textcolor{blue}{-0.4} & \textcolor{red}{+2.3} & \textcolor{red}{+1.7} & \textcolor{red}{+1.3} \\
    \bottomrule
    \end{tabular}
\end{table}


% ==========================================================================
% Ablation 2: Framework-Level
% ==========================================================================
\paragraph{Ablation Study on Verification-Driven Trajectory Construction.}

We evaluate whether adding multi-agent trajectories with explicit verification patterns improves performance. Concretely, we compare: (1)~single-agent ReAct trajectories only; and (2)~single-agent trajectories augmented with multi-agent verified trajectories.
Table~\ref{tab:framework-comparison} shows that augmented single-agent ReAct trajectories consistently improves performance across all benchmarks, with $+2.03$ average improvement. These results valid the contributions of trajectories with verification pattern.

\begin{table}[h]
    \centering
    \caption{Ablation study on verification-driven trajectory construction.}
    \label{tab:framework-comparison}
    \small
    \setlength{\tabcolsep}{3.5pt}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c c c}
    \toprule
    \textbf{Trajectory Source} & \textbf{BC-200-sample}& \textbf{BC-ZH} & \textbf{GAIA} & \textbf{xBench-DS-2505} \\
    \midrule
    Single-agent ReAct only & 13.8 & 26.8 & 57.6 & 68.3 \\
    Single-agent + Multi-agent (verified) & 14.5 & 27.0 & 62.8 & 70.3 \\
    \quad \textcolor{red}{$\Delta$ Improvement} & \textcolor{red}{+0.7} & \textcolor{red}{+0.2} & \textcolor{red}{+5.2} & \textcolor{red}{+2.0} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}


% ==========================================================================
% Ablation 3: Training
% ==========================================================================
\paragraph{Improvement of Reinforcement Learning.}

We compare the SFT checkpoint with its RL-updated counterpart under the same evaluation setup to verify the effectiveness of the RL stage. Table~\ref{tab:rl-ablation} shows consistent gains from RL across all five benchmarks. Improvements range from $+0.8$ to $+6.7$ points, with an average gain of $+2.6$ points. This confirms that RL training on our constructed challenging QA data provides robust additional optimization on top of SFT.

\begin{table}[h]
    \centering
    \caption{Contribution brought from RL training on deep research benchmarks.}
    \label{tab:rl-ablation}
    \small
    \begin{tabular}{l c c c c}
    \toprule
    \textbf{Training Stage} & \textbf{GAIA} & \textbf{xBench-DS-2505} & \textbf{BC-200-sample} & \textbf{BC-ZH} \\
    \midrule
    Marco DeepResearch (8B) SFT & 59.2 & 68.3 & 16.5 & 27.1 \\
    Marco DeepResearch (8B) RL & 61.2 & 75.0 & 17.3 & 29.3 \\
    \quad \textcolor{red}{$\Delta$ Improvement} & \textcolor{red}{+2.0} & \textcolor{red}{+6.7} & \textcolor{red}{+0.8} & \textcolor{red}{+2.2} \\
    \bottomrule
    \end{tabular}
\end{table}



% ==========================================================================
% Ablation 4: Test-Time Scaling
% ==========================================================================
\paragraph{Test-Time Scaling.}

We evaluate the effectiveness of our proposed test-time scaling strategy on the top of the RL checkpoint. Table~\ref{tab:inference-comparison} shows that our strategy delivers substantial gains at test time. Compared with the RL baseline, performance improves by $+8.7$ on GAIA, $+7.0$ on xBench-DeepSearch-2505, $+15.0$ on BrowseComp-200-sample, and $+17.8$ on BrowseComp-ZH. The average gain is $+12.1$ points, indicating the potential of our proposed test-time scaling strategy.

\begin{table}[h]
    \centering
    \caption{Contribution of our proposed verifier-guided test-time scaling.}
    \label{tab:inference-comparison}
    \small
    \setlength{\tabcolsep}{3.5pt}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l c c c c}
    \toprule
    \textbf{Inference Strategy} & \textbf{GAIA} & \textbf{xBench-DS-2505} & \textbf{BC-200-sample} & \textbf{BC-ZH} \\
    \midrule
    Marco DR (8B) SFT+RL & 61.2 & 75.0 & 17.3 & 29.3 \\
    + Discard-all & 61.5 & 72.0 & 23.7 & 38.9 \\
    %+ Verify & & & & 41.8 \\
    + Discard-all + Verify & 69.9 & 82.0 & 32.3 & 47.1 \\
    \quad \textcolor{red}{$\Delta$ vs.\ baseline} & \textcolor{red}{+8.7} & \textcolor{red}{+7.0} & \textcolor{red}{+15.0} & \textcolor{red}{+17.8} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

\paragraph{Context Window Extension during Training.}

We further study whether extending the training context window improves long-horizon deep-search performance. Using the same SFT setup, data, and evaluation protocol, we compare 64K and 128K context settings. As shown in Table~\ref{tab:context-length}, increasing the context window from 64K to 128K yields consistent gains on both benchmarks, with improvements of $+2.3$ on BrowseComp-200-sample and $+0.8$ on BrowseComp-ZH (average: $+1.6$). This result supports the importance of long-context training for deep-search tasks that require many tool calls and cross-page evidence aggregation.


\begin{table}[h]
    \centering
    \caption{Effect of extending SFT context length from 64K to 128K.}
    \label{tab:context-length}
    \small
    \begin{tabular}{l c c}
    \toprule
    \textbf{Models} & \textbf{BC-200-sample} & \textbf{BrowseComp-ZH} \\
    \midrule
    Marco DeepResearch (8B) SFT 64K & 14.2 & 26.3 \\
    Marco DeepResearch (8B) SFT 128K & 16.5 & 27.1 \\
    \quad \textcolor{red}{$\Delta$ Improvement} & \textcolor{red}{+2.3} & \textcolor{red}{+0.8} \\
    \bottomrule
    \end{tabular}
\end{table}

==> Marco_DeepResearch/sections/introduction.tex <==
% =============================================================================
% Section 1: Introduction
% =============================================================================

\section{Introduction}
\label{sec:introduction}

% ---- Figure 1: Benchmark Comparison ----
\begin{figure}[ht]
    \centering
    %\fbox{\parbox{0.95\textwidth}{\centering\vspace{4cm}\textcolor{gray}{\large\textbf{Benchmark Comparison Chart Placeholder}}\\\vspace{0.5cm}
    %\textcolor{gray}{Performance comparison across BrowseComp-EN/ZH, GAIA, HLE, WebWalkerQA, xBench}\\[4pt]
    %\textcolor{gray}{Groups: Ours \textbar{} $\leq$8B \textbar{} $>$14B \textbar{} Foundation Models}
    %\vspace{4cm}}}
    \includegraphics[width=\textwidth]{./figures/benchmark_chart_v2.pdf}
    \caption{Benchmark performance of our proposed Marco DeepResearch 8B-scale agent.}
    \label{fig:benchmark}
\end{figure}

% ---- P1: Background ----
Large language models (LLMs) have enabled tool-augmented agents that can autonomously reason and interact with external environments~\cite{team2025tongyi,huang2025deep}. Within this line, Deep research agents~\cite{OpenAI-DeepResearch, Gemini-DeepResearch} have attracted broad attention: proprietary systems such as OpenAI Deep Research~\cite{OpenAI-DeepResearch} and Gemini Deep Research~\cite{Gemini-DeepResearch} demonstrate exceptional information-seeking capabilities for solving complex tasks in real-world scenarios, while open-source systems like MiroThinker~\cite{miromind2025mirothinker}, Tongyi DeepResearch~\cite{team2025tongyi}, and AgentCPM-Explore~\cite{AgentCPMExplore2026} have rapidly narrowed the gap and in some settings matched or surpassed proprietary alternatives~\cite{mialon2023gaiabenchmarkgeneralai,wei2025browsecompsimplechallengingbenchmark,phan2025humanitysexam}. This progress is largely driven by advances in data synthesis~\cite{li2025websailornavigatingsuperhumanreasoning,tao2025webshaperagenticallydatasynthesizing}, reinforcement learning~\cite{shao2024deepseekmathpushinglimitsmathematical,dong2025agenticreinforcedpolicyoptimization}, and test-time scaling~\cite{xu2026wideseekr1exploringwidthscaling,li2025chainofagentsendtoendagentfoundation}.

% ---- P3: Core problem (concentrated definition) ----
Despite this progress, current deep research agents face a critical bottleneck: the lack of explicit verification across the following three essential stages, leading to error propagation and overall performance degradation of agents~\cite{c3b1c1524d8941978df8bd55d513abc7,lan2024traininglanguagemodelscritique,lan2024criticevalevaluatinglargelanguage}:
(1) \textbf{QA Data Synthesis}: most works synthesize QA samples from graph-based~\cite{wu2025webwalkerbenchmarkingllmsweb} or agent-based web exploration~\cite{xu2026sagesteerableagenticdata}, but entity obfuscation—the most widely adopted technique in existing pipelines—often yields non-unique or incorrect answers~\cite{meituanlongcatteam2026longcatflashthinking2601technicalreport}, undermining supervision quality and propagating errors to downstream trajectory construction; 
(2) \textbf{Trajectory construction}: most existing works rely on strong teacher models  to generate ReAct-style trajectories that can directly reach correct final answers, but these trajectories usually lack explicit verification~\cite{yao2023reactsynergizingreasoningacting}; as a result, trained agents tend to accept early low-quality results, under-explore high-value alternatives~\cite{hu2025webcotenhancingwebagent,wan2026inference}; 
and (3) \textbf{Test-time scaling}: systems generally lack explicit verification for both intermediate steps and the final answers during inference; consequently, flawed intermediate states and incorrect conclusions propagate unchecked, leading agents to accept early errors rather than triggering verifier-guided behaviors to effectively scale test-time compute~\cite{wan2026inference}.

% ---- P4: Our approach ----
To address these verification gaps, we present \textbf{Marco DeepResearch}, an efficient 8B-scale deep research agent with three improvements across these stages: (1) \textbf{Verified Data Synthesis} (Section~\ref{sec:verified-data}): where we introduce an explicit verification mechanisms to graph-based and agent-based QA synthesis methods so that question-answer pairs are carefully checked, ensuring their difficulties, uniqueness and correctness; (2) \textbf{Verification-Driven Trajectory Construction} (Section~\ref{sec:verified-framework}): where we introduce a specialized verifier agent to verify the answers of sub-tasks and final answer using web search tools, providing more explicit verification patterns into single-agent and multi-agent trajectories; and (3) \textbf{Verifier-Guided Test-Time Scaling} (Section~\ref{sec:verified-inference}): we use the Marco DeepResearch agent itself as a verifier and continue reasoning on challenging questions under a controlled compute budget, thereby more effectively unlocking the potential of test-time scaling.

% ---- P5: Contributions ----
%In summary, our main contributions are:
%\begin{itemize}[leftmargin=*, itemsep=4pt]
%\item \textbf{Verified data synthesis.}
%We introduce a verification agent to check question and answer quality in both graph-based and agent-based web random-walk QA synthesis, substantially %improving supervision quality.
%\item \textbf{Agent framework.}
%A verification-centric trajectory synthesis approach: we design a multi-agent framework with a verification sub-agent to provide explicit verification for %each sub-task and inject explicit verification patterns into final trajectories; we also re-rollout rejective-sampling-discarded trajectories via %verification and reflection to recover useful training signals.
%\item \textbf{Test-time scaling.}
%We use the base model as a verifier agent and scale inference by extending reasoning turns on hard questions, improving answer coverage without additional training.
%\item \textbf{RL optimization.}
%\textcolor{red}{[To be elaborated.]}
%\item \textbf{Data release.}
%\textcolor{gray}{[To be confirmed.]} We plan to release our verified QA datasets and trajectory data.
%\end{itemize}

% ---- P6: Results ----
With these optimizations, we synthesize high-quality trajectories and train the Marco DeepResearch agent based on the Qwen3-8B base model~\cite{yang2025qwen3technicalreport}, and evaluate it on six  deep search benchmarks like BrowseComp~\cite{wei2025browsecompsimplechallengingbenchmark}, BrowseComp-ZH~\cite{zhou2025browsecompzhbenchmarkingwebbrowsing}, and GAIA~\cite{mialon2023gaiabenchmarkgeneralai}.
Specifically, Marco DeepResearch outperforms 8B-scale deep research agents on most challenging deep benchmarks such as BrowseComp~\cite{miromind2025mirothinker,AgentCPMExplore2026}. Moreover, under a budget of up to 600 tool calls~\cite{miromind2025mirothinker}, our proposed Marco DeepResearch agent surpasses MiroThinker-v1.0-8B on BrowseComp-ZH and matches or exceeds several 30B-scale agents, including Tongyi DeepResearch-30B~\cite{team2025tongyi} and MiroThinker-v1.0-30B~\cite{miromind2025mirothinker}. Ablation studies further prove the contributions of our designs for optimizing Marco DeepResearch.


==> Marco_DeepResearch/sections/multi_agent_framework.tex <==
% =============================================================================
% Section 4: Multi-Agent Trajectory Synthesis Framework
% =============================================================================

\section{Multi-Agent Trajectory Synthesis Framework}
\label{sec:multi-agent-framework}

While Section~\ref{sec:data-synthesis} addresses the quality and diversity of QA data, this section presents our multi-agent framework for synthesizing high-quality agentic trajectories from these QA pairs.
The core insight motivating our design is that trajectories generated through multi-agent collaboration naturally encode richer behavioral patterns---including explicit task decomposition, focused sub-task execution, and systematic verification---than those produced by single-agent rollouts.

\subsection{Design Principles}
\label{sec:framework-design}

Our multi-agent trajectory synthesis framework is guided by three principles:

\paragraph{Explicit task decomposition.}
Complex research questions rarely admit direct, single-step solutions.
Effective research requires breaking down the overarching question into focused sub-problems, each amenable to targeted information retrieval.
Our framework enforces this decomposition through a dedicated planning agent, ensuring that every synthesized trajectory contains structured, hierarchical reasoning.

\paragraph{Intermediate verification.}
Errors in early reasoning steps can propagate and compound throughout a trajectory, leading to fundamentally flawed conclusions.
By introducing verification at the sub-task level---not just at the final answer---our framework catches and corrects errors early, producing trajectories that model effective self-correction behaviors.

\paragraph{Role specialization.}
Assigning distinct roles to different agents enables each to focus on its specific competency.
The planning agent can devote its full capacity to strategic reasoning, while the search agent focuses on efficient information retrieval, and the verifier agent concentrates on rigorous quality assessment.
This specialization produces trajectories with higher-quality outputs at each stage of the research process.


\subsection{Framework Architecture}
\label{sec:framework-arch}

Our framework comprises three specialized agents that collaborate to produce complete research trajectories.
The overall architecture and interaction flow are illustrated in Figure~\ref{fig:overview}.

\paragraph{Main-agent: task planning and decomposition.}
The main-agent serves as the strategic coordinator of the research process.
Given a complex question, it formulates a high-level plan by decomposing the question into a sequence of focused sub-problems.
For each sub-problem, the main-agent generates a clear, targeted query and delegates it to the search sub-agent.
Upon receiving sub-task results and verification feedback, the main-agent updates its plan, integrates partial findings, and determines the next steps.
The main-agent is also responsible for synthesizing the final answer by aggregating verified sub-task results into a coherent conclusion.
Critically, the main-agent's planning and revision behavior is explicitly recorded in the trajectory, providing the model with structured examples of strategic reasoning and adaptive replanning.

\paragraph{Search sub-agent: focused sub-task execution.}
The search sub-agent is a specialized information retrieval module that receives focused queries from the main-agent and executes targeted search operations.
For each sub-task, the sub-agent performs web searches, visits relevant pages, extracts pertinent information, and returns structured results to the main-agent.
By operating on narrow, well-defined sub-queries rather than the full research question, the sub-agent achieves more focused and efficient information retrieval, reducing the noise and irrelevant information that often plague single-agent approaches.

\paragraph{Verifier agent: quality assurance.}
The verifier agent operates as an independent third party responsible for validating the correctness and completeness of both intermediate sub-task results and the main-agent's final answer.
For each sub-task result returned by the search sub-agent, the verifier independently searches for corroborating evidence and assesses whether the result is accurate, complete, and well-supported.
If verification fails, the verifier provides detailed feedback identifying the specific issues---such as factual errors, incomplete coverage, or unsupported claims---and returns this feedback to the main-agent, triggering a revision cycle.
For the main-agent's final answer, the verifier performs a comprehensive validation before the answer is accepted.
Only answers that pass the verifier's quality gate are included in the final trajectory.

\subsection{Trajectory Generation Process}
\label{sec:framework-process}

The trajectory generation process proceeds as follows:
\begin{enumerate}[leftmargin=*, itemsep=2pt]
    \item \textbf{Initialization:} Given a question $q$ from our QA dataset (Section~\ref{sec:data-synthesis}), the main-agent analyzes the question and generates an initial plan $P = \{s_1, s_2, \ldots, s_n\}$ consisting of $n$ sub-tasks.
    \item \textbf{Sub-task execution:} For each sub-task $s_i$, the main-agent delegates a focused query to the search sub-agent, which performs information retrieval and returns results $r_i$.
    \item \textbf{Intermediate verification:} The verifier agent independently evaluates each result $r_i$. If verification succeeds, the result is accepted. If verification fails, the verifier provides feedback $f_i$, and the process returns to step 2 with a revised sub-task query informed by the feedback.
    \item \textbf{Plan revision:} After processing each sub-task, the main-agent may revise its plan based on accumulated findings, adding new sub-tasks or modifying existing ones as needed.
    \item \textbf{Answer synthesis:} Once all sub-tasks are complete, the main-agent synthesizes the final answer $a$ from the verified sub-task results.
    \item \textbf{Final verification:} The verifier agent performs a comprehensive check on the final answer. Only verified answers are accepted.
\end{enumerate}

The complete trajectory $\mathcal{T} = \{(P, s_1, r_1, v_1, f_1), \ldots, (P', s_n, r_n, v_n, f_n), a, v_{\text{final}}\}$ captures the full multi-agent interaction, including planning, execution, verification, and revision steps.
This rich structure provides the training model with explicit examples of the behavioral patterns we seek to instill: hierarchical planning, focused execution, systematic verification, and adaptive self-correction.


\subsection{Advantages over Single-Agent Synthesis}
\label{sec:framework-advantages}

Compared to single-agent trajectory synthesis, our multi-agent framework offers several key advantages:

\paragraph{Richer behavioral patterns.}
Single-agent rollouts typically produce linear interaction sequences dominated by search--observe loops with minimal planning or verification.
Our framework generates trajectories that explicitly encode task decomposition, intermediate verification, and error-driven reflection, providing the model with diverse and structured behavioral exemplars.

\paragraph{Higher trajectory quality.}
The verifier agent acts as a quality gate at multiple stages, catching errors before they propagate.
This produces trajectories where intermediate results are more accurate and final answers are more reliable, reducing the noise in training data.

\paragraph{Scalable interaction depth.}
The multi-agent structure naturally scales the depth of interaction without increasing the burden on any single agent's context window.
Complex questions that require extensive exploration can be handled by distributing the search across focused sub-tasks, each with manageable context requirements.

\paragraph{Rich behavioral patterns.}
By generating training data through multi-agent collaboration, the model learns behavioral patterns---task decomposition, intermediate verification, and error-driven re-exploration---that improve its general reasoning ability, benefiting both single-agent and multi-agent deployment scenarios.


==> Marco_DeepResearch/sections/reinforcement_learning.tex <==
% =============================================================================
% Section 6: Reinforcement Learning
% =============================================================================

\section{Reinforcement Learning}
\label{sec:rl}

After supervised fine-tuning, we further improve the agent's capabilities through reinforcement learning (RL) with environmental interaction.
This stage enables the model to explore beyond the boundaries of demonstration data and develop its own strategies for complex research tasks through trial-and-error learning.

\subsection{Problem Formulation}
\label{sec:rl-formulation}

We formulate the deep research task as a sequential decision-making problem.
Given a question $q$, the agent produces an interaction trajectory $\mathcal{H} = \{(\tau_1, a_1, o_1), \ldots, (\tau_T, a_T, o_T)\}$, where $\tau_t$ denotes the agent's reasoning at step $t$, $a_t$ denotes the action (tool call or answer generation), and $o_t$ denotes the environment observation.
The policy $\pi_\theta$ generates each thought--action pair conditioned on the trajectory history:
\begin{equation}
\tau_t, a_t \sim \pi_\theta(\cdot \mid q, \mathcal{H}_{<t}).
\end{equation}

Upon trajectory completion, a reward $R(q, \mathcal{H})$ is computed based on the correctness of the final answer.
The training objective is to find parameters $\theta^*$ that maximize the expected reward across the training distribution.


\subsection{Reward Design}
\label{sec:rl-reward}

\textcolor{red}{[To be elaborated once RL reward design is finalized.]}

We design the reward signal based on answer correctness as the primary criterion.
For questions with verifiable ground-truth answers, the reward is determined by exact or fuzzy matching against the reference answer:
\begin{equation}
R(q, \mathcal{H}) = \begin{cases} 1, & \text{if } a_T \text{ matches the ground-truth answer} \\ 0, & \text{otherwise} \end{cases}
\end{equation}

\textcolor{red}{[Potential extensions to be described: (1) verifier-based reward signals for questions without exact ground truth, (2) intermediate step rewards, (3) reward shaping for trajectory quality.]}


\subsection{Training Algorithm}
\label{sec:rl-algorithm}

\textcolor{red}{[To be elaborated once the specific RL algorithm (e.g., GRPO, PPO) and training details are finalized.]}

We employ \textcolor{red}{[algorithm name]} as our RL training algorithm, which optimizes the policy through on-policy rollouts in a real web environment.
Key design considerations include:

\paragraph{Real-world environment interaction.}
During RL training, the agent interacts with real web search engines and websites, producing authentic observation signals.
This ensures that the learned policy is directly applicable to real deployment conditions, avoiding the sim-to-real gap that arises from simulated environments~\cite{Tongyi-DeepResearch}.
% cite: Tongyi DeepResearch (environment design discussion)

\paragraph{Sandbox environment optimization.}
\textcolor{red}{[To be described: sandbox setup for safe and efficient RL training, including containerization, timeout handling, and caching mechanisms.]}

\paragraph{Training acceleration.}
\textcolor{red}{[To be described: techniques for accelerating agentic RL training, including parallel rollout, caching of search results, and efficient trajectory processing.]}

\paragraph{Long-trajectory challenges.}
Deep research tasks often produce extremely long trajectories that pose challenges for RL training in terms of both credit assignment and computational cost.
\textcolor{red}{[To be described: specific solutions for handling long trajectories, e.g., length normalization~\cite{SFR-DeepResearch}, trajectory truncation strategies, or reward denoising mechanisms~\cite{AgentCPM-Explore}.]}
% cite: SFR-DeepResearch (length-normalized RL), AgentCPM-Explore (reward denoising)


==> Marco_DeepResearch/sections/related_work.tex <==
% =============================================================================
% Section 2: Related Work
% =============================================================================

\section{Related Work}
\label{sec:related}


\paragraph{Deep Research agent systems.}


LLM-based agent systems have demonstrated profound potential and versatility across a wide spectrum of complex tasks~\cite{yang2025hscodecomprealisticexpertlevelbenchmark,lan2025deepwidesearchbenchmarkingdepthwidth,ye2026umemunifiedmemoryextraction,team2025tongyi,5team2026glm5vibecodingagentic}. Building on this foundation, \textit{Deep Research} has emerged as a frontier application, with commercial systems~\cite{OpenAI-DeepResearch,Gemini-DeepResearch} showcasing remarkable capabilities in conducting open-ended investigations and synthesizing comprehensive reports. At the very core of these sophisticated research systems lies \textit{Deep Search} (i.e., agentic information seeking)---the indispensable engine that enables agents to autonomously plan, navigate multi-turn web interactions, and extract reasoning-driven evidence~\cite{lan2025deepwidesearchbenchmarkingdepthwidth,huang2025deep,lan2026tableassearchformulatelonghorizonagentic,wong2025widesearchbenchmarkingagenticbroad}. However, despite rapid advancements and the emergence of open-source deep research agents~\cite{miromind2025mirothinker,team2025tongyi}, critical bottlenecks persist in data quality and inference-time strategies during long horizons.

%LLM-based agent systems have demonstrated broad applications and potential across diverse tasks~\cite{yang2025hscodecomprealisticexpertlevelbenchmark,lan2025deepwidesearchbenchmarkingdepthwidth,ye2026umemunifiedmemoryextraction,team2025tongyi,5team2026glm5vibecodingagentic}.
% cite: agent system survey papers
%Among these, agentic information seeking, where agents autonomously plan, search, and synthesize answers through multi-turn web interactions, has emerged as one of the most impactful and valuable applications~\cite{lan2025deepwidesearchbenchmarkingdepthwidth,huang2025deep,lan2026tableassearchformulatelonghorizonagentic,wong2025widesearchbenchmarkingagenticbroad}.
%Commercial systems~\cite{OpenAI-DeepResearch,Gemini-DeepResearch} have showcased strong capabilities on complex research tasks.
%Despite rapid advancements in the open-source community~\cite{miromind2025mirothinker,team2025tongyi}, critical bottlenecks persist in data quality and inference-time strategies.
%In the open-source community, a rapidly growing body of work has been dedicated to advancing agentic search performance~\cite{miromind2025mirothinker,team2025tongyi}. These efforts collectively advance the frontier of agentic search, yet critical challenges still remain in data quality and inference-time strategies.


\paragraph{Data synthesis for deep research agents.}
High-quality synthetic data is the key to the agentic search capabilities~\cite{team2025tongyi,hu2025stepdeepresearchtechnicalreport,tao2025webshaperagenticallydatasynthesizing}. Current approaches to agentic data synthesis mainly follow two paradigms: (1) graph-based methods traverse knowledge graphs to synthetic multi-hop QA data~\cite{miromind2025mirothinker}; (2) agent-based methods use agents explore real web environments~\cite{xu2026sagesteerableagenticdata} for data synthesis. Despite their differences, both paradigms face a common and fundamental challenge: automatically synthesizing difficult QA pairs with unique and correct answers~\cite{meituanlongcatteam2026longcatflashthinking2601technicalreport}. To address this issue, we design a verification-driven method to improve QA data quality. %that validates answer uniqueness and correctness during QA synthesis.

\paragraph{Trajectory construction.}
The ReAct paradigm~\cite{yao2023reactsynergizingreasoningacting} serves as the foundation of most current agentic systems.
Recent works have improved upon ReAct through procedural planning~\cite{wang2023planandsolvepromptingimprovingzeroshot}, multi-agent orchestration~\cite{wong2025widesearchbenchmarkingagenticbroad,lan2026tableassearchformulatelonghorizonagentic}, and context management~\cite{deepagent}.
However, these frameworks share a critical limitation: the absence of \emph{explicit verification} during interactions~\cite{wan2026inference}.
In long-horizon information seeking, agents must navigate massive search spaces where intermediate results are often noisy or misleading.
Without a dedicated verification mechanism, agents are prone to accepting the first plausible-looking answer and terminating exploration prematurely, even when the result is incorrect~\cite{wan2026inference}.
To address this limitation, we introduce an explicit verification mechanisms for both intermediate search results and final answers, designed to effectively teach the model robust verification behaviors.

\paragraph{Test-time scaling.}
At test time, deep research agents solve complex problems through extensive interactive exploration of web environments.
Effective test-time scaling strategies can significantly enhance agent performance by allocating more computation at inference~\cite{snell2024scalingllmtesttimecompute,miromind2025mirothinker,zhu2026retracrecursivetrajectorycompression,miromindteam2026mirothinker17h1heavyduty}.
While current test-time scaling approaches for agentic search primarily focus on multi-agent coordination~\cite{lan2026tableassearchformulatelonghorizonagentic} and context summarization~\cite{wu2025resumunlockinglonghorizonsearch,zhu2026retracrecursivetrajectorycompression}, the role of explicit verification as a systematic test-time scaling strategy for trained deep search agents remains largely unexplored~\cite{du2026openseekerdemocratizingfrontiersearch,wan2026inferencetimescalingverificationselfevolving}.
We address this gap by using Marco DeepResearch itself as a verifier at inference time, realizing effective test-time scaling by extending reasoning turns.


==> Marco_DeepResearch/sections/test_time_scaling.tex <==
% =============================================================================
% Section 7: Test-time Scaling and Inference Strategies
% =============================================================================

\section{Test-time Scaling and Inference Strategies}
\label{sec:test-time}

Beyond training-time improvements, we explore strategies for enhancing model performance at inference time.
We present two complementary approaches: context management for sustained long-horizon reasoning, and multi-agent inference as a novel test-time scaling paradigm.


\subsection{Context Management}
\label{sec:context-management}

Long-horizon research tasks generate extensive interaction histories that can quickly exhaust the model's context window, leading to degraded performance as critical earlier information is displaced by recent observations.
We employ context management strategies to maintain effective reasoning capacity across arbitrarily long research sessions.

\textcolor{red}{[To be elaborated once context management details are finalized. Key aspects to be described:]}

\paragraph{Dynamic context window management.}
\textcolor{red}{[Description of how the context window is dynamically managed during inference, including strategies for retaining the most informative past interactions while discarding redundant content.]}

\paragraph{Long-trajectory compression.}
\textcolor{red}{[Description of compression mechanisms for maintaining essential information from earlier interaction steps, potentially including structured state representations or summary-based approaches.]}

\paragraph{Memory management.}
\textcolor{red}{[Description of explicit memory mechanisms that allow the agent to store and retrieve key findings beyond the immediate context window.]}


\subsection{Multi-Agent Inference Strategy}
\label{sec:multi-agent-inference}

A distinctive feature of our approach is that the multi-agent training paradigm naturally enables multi-agent inference at test time.
We introduce multi-agent inference as a new dimension of test-time scaling, complementary to existing approaches based on extended reasoning chains, increased context windows, or best-of-N sampling.

\paragraph{Motivation.}
Existing test-time scaling methods primarily operate along a single axis: allocating more computation to a single model instance, whether through longer reasoning chains~\cite{MiroThinker}, extended context windows, or multiple independent sampling attempts.
% cite: MiroThinker (interactive scaling)
While effective, these approaches are fundamentally limited by the single agent's capacity to simultaneously manage planning, execution, and verification within one decision-making loop.
We observe that our multi-agent training data (Section~\ref{sec:multi-agent-framework}) encodes structured patterns of task decomposition, focused execution, and systematic verification.
If the model has effectively learned these patterns during training, it should be possible to leverage them at inference time by deploying the same multi-agent collaboration structure used during data synthesis.

\paragraph{Multi-agent inference architecture.}
At inference time, we deploy the trained model in a multi-agent configuration that mirrors the training data generation process:
\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item The \textbf{main-agent} receives the user's question and generates a high-level plan by decomposing it into focused sub-tasks. It coordinates the overall research process and synthesizes the final answer.
    \item The \textbf{search sub-agent(s)} receive individual sub-task queries from the main-agent and perform focused information retrieval. Multiple sub-agents can operate in parallel on different sub-tasks, improving efficiency.
    \item The \textbf{verifier agent} validates intermediate results and the final answer, triggering revision when verification fails.
\end{itemize}

The key insight is that a single backbone model can fulfill all three roles through appropriate prompting and context configuration, as the model has been trained on trajectories containing all three behavioral patterns.

\paragraph{Training-inference consistency.}
The effectiveness of multi-agent inference rests on the principle of training-inference consistency: the model performs best when the inference paradigm aligns with the paradigm under which training data was generated.
Since our training trajectories encode explicit patterns of task decomposition (main-agent behavior), focused retrieval (sub-agent behavior), and quality verification (verifier behavior), the model can leverage these internalized patterns most effectively when deployed in a matching multi-agent configuration.
This contrasts with single-agent inference, where the model must simultaneously exhibit all these behaviors within a single decision loop, potentially conflating or under-utilizing the specialized patterns learned during training.


\paragraph{Advantages.}
Multi-agent inference offers several benefits over single-agent deployment:
(1) \textit{Structured task decomposition}---the main-agent can focus entirely on strategic planning without being interrupted by search operations;
(2) \textit{Parallel execution}---multiple sub-agents can work on different sub-tasks simultaneously, improving throughput;
(3) \textit{Systematic quality control}---the verifier agent provides an independent check at each stage, preventing error propagation;
and (4) \textit{Context efficiency}---each agent maintains a focused context relevant to its role, avoiding context dilution that occurs when a single agent must track all aspects simultaneously.


\subsection{Other Test-time Scaling Methods}
\label{sec:other-test-time}

\textcolor{red}{[To be elaborated once additional test-time scaling strategies are finalized. Potential content includes:]}

\textcolor{red}{[Best-of-N sampling with verifier-based selection, where the verifier agent scores multiple candidate answers and selects the most reliable one.]}

\textcolor{red}{[Adaptive computation allocation, where the inference budget (number of tool calls, search depth) is dynamically adjusted based on question difficulty or the model's confidence level.]}


==> Marco_DeepResearch/sections/training_pipeline.tex <==
% =============================================================================
% Section 6: Training Pipeline
% =============================================================================

\section{Training Pipeline}
\label{sec:training}

The training pipeline consists of Supervised Fine-Tuning and Reinforcement Learning.


\subsection{Supervised Fine-Tuning}
\label{sec:training-sft}

\paragraph{Training objective.}
We train with token-level cross-entropy and apply a loss mask so that only assistant response tokens contribute to optimization $\mathcal{L}_{\text{SFT}}(\theta) = - \sum_{t=1}^{T} m_t \log P_\theta(x_t \mid x_{<t})$, where the mask is defined as
\begin{equation}
m_t=
\begin{cases}
1, & t \in \mathcal{T}_{\text{assistant}},\\
0, & t \in \mathcal{T}_{\text{instruction}} \cup \mathcal{T}_{\text{tool\_response}}.
\end{cases}
\end{equation}
That is, instruction and tool response content are masked out.


\subsection{Reinforcement Learning}
\label{sec:training-rl}

Starting from the SFT checkpoint, we optimize the policy with Group Relative Policy Optimization (GRPO)~\cite{shao2024deepseekmathpushinglimitsmathematical}, where updates are driven by within-group relative advantages. Concretely, for each query $q$, we sample a group of $G$ rollouts $\{o_i\}_{i=1}^{G}$ from the old policy $\pi_{\theta_{\text{old}}}$ and optimize
\iffalse
\begin{equation}
\mathcal{J}_{\text{GRPO}}(\theta)=
\mathbb{E}_{q\sim P(Q),\,\{o_i\}_{i=1}^{G}\sim \pi_{\theta_{\text{old}}}(\cdot|q)}
\left[
\frac{1}{G}\sum_{i=1}^{G}
\min\!\left(
\frac{\pi_{\theta}(o_i|q)}{\pi_{\theta_{\text{old}}}(o_i|q)}\hat{A}_i,\,
\mathrm{clip}\!\left(\frac{\pi_{\theta}(o_i|q)}{\pi_{\theta_{\text{old}}}(o_i|q)},1-\epsilon,1+\epsilon\right)\hat{A}_i
\right)
- \beta\, \mathbb{D}_{\text{KL}}\!\left[\pi_{\theta} \,\|\, \pi_{\text{ref}}\right]
\right]
\end{equation}
\fi
\begin{equation}
\begin{aligned}
\mathcal{J}_{\text{GRPO}}(\theta) = \mathbb{E}_{\substack{q \sim P(Q) \\ \{o_i\}_{i=1}^{G} \sim \pi_{\theta_{\text{old}}}}} \Bigg[ & \frac{1}{G}\sum_{i=1}^{G} \min \Big( r_i(\theta)\hat{A}_i,\, \mathrm{clip}\!\left(r_i(\theta), 1-\epsilon, 1+\epsilon\right)\hat{A}_i \Big) \\
& - \beta\, \mathbb{D}_{\text{KL}}\!\left[\pi_{\theta} \,\|\, \pi_{\text{ref}}\right] \Bigg]
\end{aligned}
\end{equation}
where $r_i(\theta) = \frac{\pi_{\theta}(o_i|q)}{\pi_{\theta_{\text{old}}}(o_i|q)}$ denotes the importance sampling ratio. The relative advantage is computed by reward normalization within each group:
\begin{equation}
\hat{A}_i = \frac{r_i - \mathrm{mean}\left(\{r_j\}_{j=1}^{G}\right)}{\mathrm{std}\left(\{r_j\}_{j=1}^{G}\right)}.
\end{equation}
%The relative advantage is computed by reward normalization within each group:
%\begin{equation}
%\hat{A}_i=\frac{r_i-\mathrm{mean}(\{r_j\}_{j=1}^{G})}{\mathrm{std}(\{r_j\}_{j=1}^{G})}.
%\end{equation}

We adopt an outcome-based reward, and balance reward quality and computational cost by using a two-stage LLM-as-Judge pipeline: a fast primary judge (Qwen-Turbo-Latest) evaluates all samples, and uncertain or low-confidence cases are escalated to a secondary judge (GPT-4.1) for re-evaluation:
\begin{equation}
r(q,o)=
\begin{cases}
1, & \text{if }\mathcal{J}(o,a^{*})=\text{correct},\\
0, & \text{otherwise},
\end{cases}
\end{equation}
where $q$ is the input query, $o$ is the generated output, $a^{*}$ is the reference answer, and $\mathcal{J}(\cdot)$ is the judging function.

==> Marco_DeepResearch/sections/trajectory_optimization.tex <==
% =============================================================================
% Section 5: Trajectory Optimization
% =============================================================================

\section{Trajectory Optimization}
\label{sec:trajectory-optimization}

Not all trajectories generated by the multi-agent framework succeed in reaching the correct answer.
Rather than discarding these erroneous trajectories, we argue that they contain valuable learning signals: failed trajectories reveal common failure modes, identify challenging sub-problems, and provide natural starting points for injecting self-reflection behaviors.
In this section, we introduce two complementary trajectory optimization strategies that transform erroneous trajectories into effective training resources.

\subsection{Motivation}
\label{sec:traj-opt-motivation}

Erroneous trajectories are a natural byproduct of any data synthesis pipeline, and their prevalence increases with question difficulty.
We observe that these trajectories, while incorrect in their final answers, often contain partially correct reasoning chains, useful intermediate findings, and informative failure points.
Discarding them entirely wastes a substantial fraction of synthesis effort and, more importantly, forfeits the opportunity to teach the model \textit{how to recover from mistakes}---a capability that is critical for robust research agents.

Our trajectory optimization strategy explicitly injects self-reflection patterns into the training data, teaching the model to recognize its own errors and revise its approach.
This strategy leverages the verifier agent (Section~\ref{sec:framework-arch}) to identify which trajectories require optimization and to guide the recovery process.


\subsection{Reflection-Guided Re-rollout}
\label{sec:traj-reflection}

We explicitly inject self-reflection patterns into the model's behavioral repertoire through reflection-guided re-rollout.

\paragraph{Core idea.}
Given an erroneous trajectory $\mathcal{T}^-$ for question $q$, we construct a \textit{reflection-augmented trajectory} that demonstrates the process of recognizing an error, reflecting on its cause, and successfully revising the approach.
This provides the model with explicit training examples of the self-correction behavior that is largely absent from standard trajectory data.

\paragraph{Reflection and re-rollout process.}
The process operates in three steps:
\begin{enumerate}[leftmargin=*, itemsep=2pt]
    \item \textbf{Error identification:} The verifier agent analyzes the erroneous trajectory $\mathcal{T}^-$ and identifies the specific point(s) of failure, producing a structured error analysis that pinpoints incorrect reasoning steps or faulty information retrieval.
    \item \textbf{Reflection generation:} Based on the error analysis, a reflection segment is generated that explicitly articulates: (a) what went wrong in the original approach, (b) why the error occurred, and (c) what alternative strategy should be adopted. This reflection is appended to the trajectory context.
    \item \textbf{Re-rollout:} Starting from the reflection, the agent re-executes the research process with the revised strategy, producing a new trajectory segment. If the re-rollout reaches the correct answer, the complete sequence---original attempt, error identification, reflection, and successful revision---forms a reflection-augmented training example.
\end{enumerate}

\paragraph{Training with reflection data.}
The reflection-augmented trajectories are incorporated into the SFT training set, providing the model with explicit demonstrations of the think--reflect--revise cycle.
This approach directly injects the self-reflection behavioral pattern that we identified as lacking in existing trajectory data (Section~\ref{sec:introduction}).

The reflection-augmented trajectories equip the model with the practical skill of self-correction---recognizing errors and revising strategies---a capability that is largely absent from standard trajectory data. The effectiveness of this approach is validated by our analysis experiments in Section~\ref{sec:experiments}.


==> Marco_DeepResearch/sections/verified_data.tex <==
% =============================================================================
% Section 3: Verified Data Synthesis
% =============================================================================

\section{Verified Data Synthesis}
\label{sec:verified-data}

In this section, we apply explicit verification to QA data synthesis to ensure the quality and answer uniqueness while keeping their difficulties.
High-quality QA data is essential for both trajectory synthesis and optimization.
A common bottleneck in existing approaches is \textit{answer non-uniqueness}: to increase question difficulty, most methods obfuscate entity information in multi-hop questions~\cite{miromind2025mirothinker, xu2026sagesteerableagenticdata}, which inevitably introduces ambiguity and may result in low-quality questions with multiple valid answers.
When such data is used as ground truth, the training becomes biased and unstable.
We address this problem through two complementary synthesis pipelines: graph-based and agent-based, each incorporating explicit verification to guarantee answer quality.

% ---- Figure 2: Framework Overview ----
\begin{figure*}[t]
    %\centering
    %\fbox{\parbox{0.95\textwidth}{\centering\vspace{4cm}\textcolor{gray}{\large\textbf{Framework Overview Placeholder}}\\\vspace{0.5cm}
    %\textcolor{gray}{Level 1: Verified Data Synthesis (Graph-based + Agent-based QA)}\\[4pt]
    %\textcolor{gray}{Level 2: Agent Framework (Single-Agent ReAct + Multi-Agent with Verification)}\\[4pt]
    %\textcolor{gray}{Level 3: Test-Time Scaling (Re-rollout Strategies)}\\[4pt]
    %\textcolor{gray}{Bottom: Training Pipeline (SFT $\rightarrow$ RL)}
    %\vspace{4cm}}}
    \includegraphics[width=\textwidth]{./figures/figure1_design.pdf}
    \caption{Overall framework of our verification-center design for Marco DeepResearch agents.}
    \label{fig:overview}
\end{figure*}

%\subsection{QA Data Verification}
%\label{sec:qa-verification}


\subsection{Graph-Based Synthesis with Adversarial Verification}
\label{sec:qa-graph}

Most graph-based QA synthesis methods still face a core difficulty: it is hard to jointly guarantee search depth, answer uniqueness, correctness, and entity leakage control in QA construction~\cite{meituanlongcatteam2026longcatflashthinking2601technicalreport}. To address this, we introduce a unified paradigm of \textit{answer-first reverse construction with adversarial verification} in graph-based QA synthesis, organized as an iterative loop:

\paragraph{Answer entity sampling.}
We first sample answer entities under structural and content constraints on knowledge-graph (e.g., moderate connectivity, sufficient document evidence, and valid predecessor nodes), ensuring tasks necessitate multi-hop reasoning while avoiding trivial common-knowledge shortcuts.

\paragraph{Structured attribute profiling.}
Given documents linked to the each sampled answer entity, we leverage frontier models to extract a structured attribute profile over five dimensions: spatial, temporal, numerical, categorical, and entity-relation features. This profile provides the candidate constraints for controlled obfuscation and question construction.

\paragraph{Reverse path search.}
Starting from the selected answer entity, we search backward for intermediate evidence nodes using complementary graph-structure search and content-matching search (attribute keywords matching). Then, strong LLMs are used to select a small set of high-quality, diverse intermediates (4 to 8 intermediates) to form a robust multi-hop reasoning chain.

\paragraph{Adversarial answer uniqueness verification.}
After getting a searched path containing the answer entity, we apply an adversarial verification process to ensure answer uniqueness. This is the key verification process to ensure answer uniqueness and difficulty of synthesized QA pairs, which is an iterative three-role process with a \textit{Generator}, an \textit{Attacker}, and an \textit{Analyzer}. 
The Generator first initializes 2--3 obfuscated constraints from the attribute profile; the Attacker then searches for counterexample entities that satisfy all current constraints but are not the target answer. If no counterexample is found and the constraint count is above a minimum threshold, the loop converges; otherwise, the Analyzer adds new discriminative constraints and returns control to the Attacker.
This loop runs for at most 10 rounds. Its convergence follows a monotonicity principle: each round appends at least one new constraint, and each added constraint removes at least part of the counterexample set. As a result, the final constraint set provides high-confidence answer uniqueness for the target entity.

Finally, after convergence, we convert constraints into natural-language multi-hop questions and apply leakage checks to obscure key entities. Samples exhibiting leakage, or those solvable by frontier models without search and consistency checks, are excluded from our training set.


\subsection{Agent-Based Web Exploration Synthesis}
\label{sec:qa-agent}

Compared with graph-based methods, agent-based QA synthesis significantly enhances data realism and broadens domain coverage~\cite{miromind2025mirothinker,xu2026sagesteerableagenticdata}. Motivated by these advantages, we also construct QA data via agent-based web exploration, empowering agents to autonomously navigate real-world web environments to formulate real-world, complex, multi-hop questions~\cite{xu2026sagesteerableagenticdata, tao2025webshaperagenticallydatasynthesizing}. Despite its benefits, this dynamic setting inevitably introduces common failure cases, such as factual hallucinations, ambiguous answers, and pseudo multi-hop questions that are easily bypassed by shortcut retrieval~\cite{xu2026sagesteerableagenticdata}.
To control these failures, we design a Generation--Execution--Verification loop with a question agent, a search agent, and a verification agent. The key design is to separate question construction from independent solving and then enforce strict third-party verification before data acceptance.

\paragraph{Evidence-first question construction.}
Instead of forward generation, question agent first explores the open web to build an evidence graph, and constructs questions from verified evidence. During construction, it applies entity obfuscation and diverse reasoning topologies (e.g., convergent and conjunctive constraints) to reduce one-step shortcut matching while controlling target difficulty~\cite{xu2026sagesteerableagenticdata}.

\paragraph{Multi-stage quality verification.}
We employ a multi-stage filtering pipeline: a verification agent ensures factual consistency and evidence grounding, while a closed-book filter excludes questions solvable without retrieval. Remaining candidates are solved by an independent search agent, with final verification confirming reasoning depth aligns with target difficulty and no alternative valid answers satisfy the constraints~\cite{xu2026sagesteerableagenticdata}.

%For each candidate QA pair, verification agent first verifies factual consistency and evidence grounding, filtering out samples with hallucinated premises or unsupported answers. It then applies a closed-book filter: if an advanced reasoning model can answer the question without retrieval, the sample is treated as low-value and sent back for revision. For candidates that pass these gates, search agent performs independent web-based solving under context isolation from generation, and verification agent checks two final properties: (1) the observed minimum reasoning depth is consistent with the target difficulty and (2) no alternative valid answer satisfies the full constraint set~\cite{xu2026sagesteerableagenticdata}.

\paragraph{Diagnosis Iterative Optimization.}
When a sample fails at any stage, we do not simply discard it. Instead, verification agent provides structured diagnostic feedback (e.g., under-constrained question, shortcut path, insufficient depth, or evidence conflict), and question agent performs targeted updates on evidence selection, constraint design, and question structure. This diagnosis--revision loop continues until the sample jointly satisfies groundedness, uniqueness, and empirical difficulty requirements, improving data efficiency while maintaining strict quality control.

We combine the above two pipelines with additional synthesis strategies to maximize data diversity across problem types, domains, and difficulty levels. To validate data quality, we manually reviewed 100 samples. Fewer than 10\% had clear question-answer mismatch, while the remaining QA samples are valid but challenging. This result shows that our proposed methods could generate high-quality and challenging dataset for optimizing agents.

==> Marco_DeepResearch/sections/verified_framework.tex <==
% =============================================================================
% Section 4: Verified Trajectory Framework
% =============================================================================

\section{Verification-Driven Trajectory Construction}
\label{sec:verified-framework}

Single-agent ReAct is still the dominant trajectory synthesis recipe in current deep research systems~\cite{li2025websailornavigatingsuperhumanreasoning,miromind2025mirothinker}. However, this pipeline typically does not explicitly verify key intermediate results, so errors made in early steps can directly propagate and accumulate, degrading final performance. We therefore argue that high-quality trajectories should contain explicit verification patterns, including both intermediate checks for sub-task outputs and final checks for the proposed answer. Prior work~\cite{wan2026inferencetimescalingverificationselfevolving} on deep-search benchmarks also suggests that, for needle-in-a-haystack tasks, direct solving is difficult while answer verification conditioned on the question (or sub-question) is relatively reliable~\cite{mialon2023gaiabenchmarkgeneralai,wei2025browsecompsimplechallengingbenchmark}.
To capitalize on this easy-to-verify property, we introduce two complementary designs for trajectory construction: multi-agent verified synthesis and verification-reflection re-rollout.

\paragraph{Multi-agent with Verification.}
As shown in Figure~\ref{fig:overview}, we design a three-role framework with a main agent, a search sub-agent, and a verifier sub-agent. The main agent decomposes a complex problem into sub-tasks and aggregates sub-results into a final answer. The search sub-agent solves each sub-task. The verifier agent then performs independent third-party validation with web tools for both sub-task outputs and the final proposed answer. If verification fails, the corresponding step is revised and re-executed, so trajectories explicitly record verification-driven correction behavior.
Finally, the multi-agent trajectories are converted into a single-agent ReAct-style trajectories for training~\cite{li2025chainofagentsendtoendagentfoundation}.

\paragraph{Verification-Reflection Re-rollout on Failed Trajectories.}
We also collect trajectories with incorrect final answers and invoke a verifier agent to diagnose failure causes and produce actionable feedback~\cite{zhu2026retracrecursivetrajectorycompression}. Conditioned on this feedback, we re-rollout the failed trajectories and keep trajectories that are recovered to correct answers.


==> Marco_DeepResearch/sections/verified_inference.tex <==
% =============================================================================
% Section 5: Test-Time Scaling
% =============================================================================

\section{Verifier-Guided Test-Time Scaling}
\label{sec:verified-inference}

Current test-time scaling for deep research agents mainly increases interaction rounds or rollout budget~\cite{miromind2025mirothinker}. While this can improve coverage, blindly scaling turns often accumulates early tool errors and noisy intermediate conclusions, which reduces reliability on long-horizon search tasks~\cite{miromindteam2026mirothinker17h1heavyduty}. Therefore, we propose \textbf{Verifier-Guided Test-time Scaling} that adds explicit verification into inference-time scaling and uses Marco DeepResearch itself as a verifier. By combining the \textit{Discard All} context management strategy with verification~\cite{deepseekai2025deepseekv32pushingfrontieropen}, we realize more effective test-time scaling under a fixed maximum interaction budget $T_{\max}$.

\paragraph{Discard All.}
During a rollout, once predefined degeneration signals are triggered (e.g., reaching max steps or failing to solve questions), we apply \textit{Discard All} context management strategy: remove accumulated tool-call history and intermediate reasoning outputs, keep only the original query and the system prompt, and restart from a fresh context. This reset mechanism allows the agent to explore new search paths and reducing error propagation along a single trajectory~\cite{deepseekai2025deepseekv32pushingfrontieropen}.

\paragraph{Verifier-Guided Test-time Scaling.}
Whenever the agent produces a candidate answer, we conduct rule-based checks and agent-as-a-judge using Marco DeepResearch~\cite{wan2026inferencetimescalingverificationselfevolving,zhuge2024agentasajudgeevaluateagentsagents}. If $t<T_{\max}$~\cite{miromind2025mirothinker,chen2026searchmorethinkless}, the agent can continue exploring and propose additional candidates; each candidate is verified independently. When $t=T_{\max}$ or the process reaches a convergence condition, we perform \textit{Joint Verify} over all candidates and generate the final answer for the question.

These two components are complementary: \textit{Discard All} improves trajectory quality by resetting degraded contexts, while \textit{Verifier-guided Test-time Scaling} improves answer quality. Together, they realize more effective test-time scaling without changing model parameters, and unlock stronger inference-time gains on hard questions.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/abstract.tex <==
% =============================================================================
% Abstract
% =============================================================================
% NOTE: The abstract is now defined in main.tex (before \begin{document})
% as required by the paper_improved.cls template.
% This file is kept for reference only.
% =============================================================================


==> sections/data_synthesis.tex <==
% =============================================================================
% Section 3: Enhanced Data Synthesis (QA Data Synthesis)
% =============================================================================

\section{Enhanced Data Synthesis}
\label{sec:data-synthesis}

High-quality question--answer (QA) data forms the foundation for training deep research agents.
In this section, we present our enhanced data synthesis pipeline, which addresses the limitations of existing approaches in terms of quality, realism, difficulty, and diversity.

\subsection{Problem Analysis}
\label{sec:data-problem}

We identify three primary limitations of current QA data synthesis methods for deep research agent training:

\paragraph{Insufficient realism.}
Knowledge-graph-based synthesis methods~\cite{KG-QA-synthesis-refs} construct questions by composing entities and relations from structured knowledge bases.
% cite: knowledge-graph-based QA synthesis papers
While this produces questions with verifiable answers, the resulting queries often fail to reflect real-world information-seeking scenarios.
Questions derived from static knowledge graphs (e.g., those built from Wikipedia) are frequently anchored to a fixed temporal snapshot and may be trivially resolvable through alternative web sources, undermining their value as training signals for agents that must operate in dynamic, open-ended web environments.

\paragraph{Unreliable quality.}
Approaches that synthesize questions through real web exploration~\cite{SAGE} improve authenticity but introduce quality concerns.
% cite: SAGE
Without rigorous verification, synthesized answers may contain hallucinations, be non-unique across different web sources, or fail to meet the expected level of specificity and factual precision.
The open-ended nature of web information makes automated quality control inherently challenging, leading to noisy training signals that can degrade model performance.

\paragraph{Limited diversity.}
Most existing pipelines employ a single synthesis strategy, which inherently limits the diversity of the resulting dataset along multiple dimensions: problem type (factual retrieval vs.\ multi-step reasoning vs.\ analytical comparison), difficulty level (simple lookups vs.\ complex multi-hop chains), domain coverage (science, history, finance, etc.), and required reasoning patterns.
This lack of diversity constrains the model's ability to generalize across the broad spectrum of research scenarios encountered in practice.


\subsection{Knowledge-Graph-Augmented Real Web Exploration}
\label{sec:data-graph-web}

To simultaneously address realism and difficulty, we combine knowledge graph construction with real web exploration.
Our approach draws inspiration from existing graph-based and web-based methods~\cite{Step-DeepResearch, MiroThinker} while introducing key enhancements.
% cite: Step-DeepResearch (real web grounding), MiroThinker (MultiDocQA synthesis)

\paragraph{Graph construction with web grounding.}
We begin by constructing knowledge graphs from diverse, high-quality sources including encyclopedias, academic repositories, and curated web collections.
For each entity node in the graph, we perform real web exploration to identify and associate relevant web pages, grounding the abstract graph structure in authentic, accessible web content.
This web-grounding step serves two purposes: it ensures that the resulting questions require genuine web-based information seeking to resolve, and it anchors the questions in the current state of the web rather than a static knowledge snapshot.

\paragraph{Difficulty control.}
We implement explicit difficulty control mechanisms to produce questions spanning a range of complexity levels.
Specifically, we vary the number of reasoning hops required, the degree of constraint obfuscation applied to entity references, and the diversity of source domains that must be integrated.
\textcolor{red}{[To be elaborated with specific difficulty control parameters and examples.]}

\paragraph{Timeliness and authenticity.}
By associating graph nodes with real web pages and validating question answerability against live web content, our pipeline ensures that synthesized questions reflect current web conditions.
This addresses a key weakness of purely graph-based methods, where temporal drift between graph construction and model deployment can render questions unrealistic.



\subsection{Three-Agent QA Verification Framework}
\label{sec:data-verification}

To ensure the quality and factual reliability of synthesized QA pairs, we introduce a dedicated three-agent verification framework.
Unlike single-pass generation approaches, our framework employs specialized agents that independently validate different aspects of data quality.

\paragraph{Question agent.}
The question agent is responsible for generating complex, multi-hop questions by exploring real web environments and synthesizing information across multiple sources.
It produces candidate questions along with preliminary answers derived from the explored web content.
The question agent is instructed to generate questions that require genuine multi-step reasoning and cannot be resolved through simple keyword matching or single-source retrieval.

\paragraph{Search agent.}
The search agent independently attempts to solve each generated question using the available tool suite (web search, page visits, etc.).
This independent solution attempt serves as a validation mechanism: if the search agent can reliably arrive at the same answer through an independent search process, the question--answer pair is more likely to be well-formed and unambiguous.
The search agent's trajectory also provides valuable signal about the difficulty and solvability of the question.

\paragraph{Verifier agent.}
The verifier agent performs rigorous quality control by independently examining both the question and the candidate answers.
Its verification encompasses multiple dimensions:
\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textbf{Answer correctness:} The verifier cross-checks the proposed answer against independently retrieved evidence, ensuring factual accuracy.
    \item \textbf{Hallucination detection:} The verifier identifies cases where the proposed answer cannot be substantiated by available web evidence, flagging potential hallucinations.
    \item \textbf{Answer uniqueness:} The verifier checks whether alternative valid answers exist, filtering out questions with ambiguous or non-unique solutions.
    \item \textbf{Quality gate:} Questions that fail any verification criterion are either revised (with feedback from the verifier guiding the revision) or discarded, ensuring that only high-quality QA pairs enter the training set.
\end{itemize}

This three-agent verification framework provides controllable quality assurance that is difficult to achieve through single-model generation, as each agent brings an independent perspective that helps identify and eliminate different categories of errors.


\subsection{Diverse Data Synthesis Strategies}
\label{sec:data-diversity}

We argue that data diversity is as important as data quality for training robust deep research agents.
Rather than relying on a single synthesis method, we employ multiple complementary strategies, each contributing unique characteristics to the overall training set.

\paragraph{Multiple synthesis approaches.}
Our data synthesis pipeline incorporates several complementary strategies:
\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textbf{Knowledge-graph-based synthesis:} Produces structured multi-hop questions with well-defined reasoning chains, particularly effective for questions requiring integration of facts across multiple entities and relations.
    \item \textbf{Real web exploration-based synthesis:} Generates questions grounded in authentic web content, capturing the characteristics of real-world information-seeking tasks including temporal sensitivity and source diversity.
    \item \textbf{Sub-task decomposition-based synthesis:} Creates complex questions by composing multiple simpler sub-tasks, each requiring different types of information retrieval or reasoning, resulting in questions that demand structured problem-solving approaches.
    \item \textbf{Hybrid strategies:} Combines elements from the above approaches to produce questions that exhibit characteristics of multiple categories simultaneously.
\end{itemize}

\paragraph{Diversity along multiple dimensions.}
By combining these strategies, our synthesized dataset achieves diversity along four key dimensions:
(1) \textit{problem type diversity}---spanning factual retrieval, multi-step reasoning, comparative analysis, and temporal queries;
(2) \textit{difficulty gradient diversity}---ranging from straightforward lookups to complex chains requiring deep exploration;
(3) \textit{domain coverage diversity}---encompassing science, technology, history, finance, law, culture, and other areas;
and (4) \textit{trajectory pattern diversity}---reflecting different search strategies, reasoning paths, and interaction depths.

\paragraph{Empirical evidence for complementarity.}
\textcolor{red}{[To be filled with experimental evidence showing that each synthesis strategy contributes additive performance gains, and that the combined dataset outperforms any single-strategy dataset. This will be cross-referenced with the analysis experiments in Section~\ref{sec:experiments}.]}


==> sections/multi_agent_framework.tex <==
% =============================================================================
% Section 4: Multi-Agent Trajectory Synthesis Framework
% =============================================================================

\section{Multi-Agent Trajectory Synthesis Framework}
\label{sec:multi-agent-framework}

While Section~\ref{sec:data-synthesis} addresses the quality and diversity of QA data, this section presents our multi-agent framework for synthesizing high-quality agentic trajectories from these QA pairs.
The core insight motivating our design is that trajectories generated through multi-agent collaboration naturally encode richer behavioral patterns---including explicit task decomposition, focused sub-task execution, and systematic verification---than those produced by single-agent rollouts.

\subsection{Design Principles}
\label{sec:framework-design}

Our multi-agent trajectory synthesis framework is guided by three principles:

\paragraph{Explicit task decomposition.}
Complex research questions rarely admit direct, single-step solutions.
Effective research requires breaking down the overarching question into focused sub-problems, each amenable to targeted information retrieval.
Our framework enforces this decomposition through a dedicated planning agent, ensuring that every synthesized trajectory contains structured, hierarchical reasoning.

\paragraph{Intermediate verification.}
Errors in early reasoning steps can propagate and compound throughout a trajectory, leading to fundamentally flawed conclusions.
By introducing verification at the sub-task level---not just at the final answer---our framework catches and corrects errors early, producing trajectories that model effective self-correction behaviors.

\paragraph{Role specialization.}
Assigning distinct roles to different agents enables each to focus on its specific competency.
The planning agent can devote its full capacity to strategic reasoning, while the search agent focuses on efficient information retrieval, and the verifier agent concentrates on rigorous quality assessment.
This specialization produces trajectories with higher-quality outputs at each stage of the research process.


\subsection{Framework Architecture}
\label{sec:framework-arch}

Our framework comprises three specialized agents that collaborate to produce complete research trajectories.
The overall architecture and interaction flow are illustrated in Figure~\ref{fig:overview}.

\paragraph{Main-agent: task planning and decomposition.}
The main-agent serves as the strategic coordinator of the research process.
Given a complex question, it formulates a high-level plan by decomposing the question into a sequence of focused sub-problems.
For each sub-problem, the main-agent generates a clear, targeted query and delegates it to the search sub-agent.
Upon receiving sub-task results and verification feedback, the main-agent updates its plan, integrates partial findings, and determines the next steps.
The main-agent is also responsible for synthesizing the final answer by aggregating verified sub-task results into a coherent conclusion.
Critically, the main-agent's planning and revision behavior is explicitly recorded in the trajectory, providing the model with structured examples of strategic reasoning and adaptive replanning.

\paragraph{Search sub-agent: focused sub-task execution.}
The search sub-agent is a specialized information retrieval module that receives focused queries from the main-agent and executes targeted search operations.
For each sub-task, the sub-agent performs web searches, visits relevant pages, extracts pertinent information, and returns structured results to the main-agent.
By operating on narrow, well-defined sub-queries rather than the full research question, the sub-agent achieves more focused and efficient information retrieval, reducing the noise and irrelevant information that often plague single-agent approaches.

\paragraph{Verifier agent: quality assurance.}
The verifier agent operates as an independent third party responsible for validating the correctness and completeness of both intermediate sub-task results and the main-agent's final answer.
For each sub-task result returned by the search sub-agent, the verifier independently searches for corroborating evidence and assesses whether the result is accurate, complete, and well-supported.
If verification fails, the verifier provides detailed feedback identifying the specific issues---such as factual errors, incomplete coverage, or unsupported claims---and returns this feedback to the main-agent, triggering a revision cycle.
For the main-agent's final answer, the verifier performs a comprehensive validation before the answer is accepted.
Only answers that pass the verifier's quality gate are included in the final trajectory.

\subsection{Trajectory Generation Process}
\label{sec:framework-process}

The trajectory generation process proceeds as follows:
\begin{enumerate}[leftmargin=*, itemsep=2pt]
    \item \textbf{Initialization:} Given a question $q$ from our QA dataset (Section~\ref{sec:data-synthesis}), the main-agent analyzes the question and generates an initial plan $P = \{s_1, s_2, \ldots, s_n\}$ consisting of $n$ sub-tasks.
    \item \textbf{Sub-task execution:} For each sub-task $s_i$, the main-agent delegates a focused query to the search sub-agent, which performs information retrieval and returns results $r_i$.
    \item \textbf{Intermediate verification:} The verifier agent independently evaluates each result $r_i$. If verification succeeds, the result is accepted. If verification fails, the verifier provides feedback $f_i$, and the process returns to step 2 with a revised sub-task query informed by the feedback.
    \item \textbf{Plan revision:} After processing each sub-task, the main-agent may revise its plan based on accumulated findings, adding new sub-tasks or modifying existing ones as needed.
    \item \textbf{Answer synthesis:} Once all sub-tasks are complete, the main-agent synthesizes the final answer $a$ from the verified sub-task results.
    \item \textbf{Final verification:} The verifier agent performs a comprehensive check on the final answer. Only verified answers are accepted.
\end{enumerate}

The complete trajectory $\mathcal{T} = \{(P, s_1, r_1, v_1, f_1), \ldots, (P', s_n, r_n, v_n, f_n), a, v_{\text{final}}\}$ captures the full multi-agent interaction, including planning, execution, verification, and revision steps.
This rich structure provides the training model with explicit examples of the behavioral patterns we seek to instill: hierarchical planning, focused execution, systematic verification, and adaptive self-correction.


\subsection{Advantages over Single-Agent Synthesis}
\label{sec:framework-advantages}

Compared to single-agent trajectory synthesis, our multi-agent framework offers several key advantages:

\paragraph{Richer behavioral patterns.}
Single-agent rollouts typically produce linear interaction sequences dominated by search--observe loops with minimal planning or verification.
Our framework generates trajectories that explicitly encode task decomposition, intermediate verification, and error-driven reflection, providing the model with diverse and structured behavioral exemplars.

\paragraph{Higher trajectory quality.}
The verifier agent acts as a quality gate at multiple stages, catching errors before they propagate.
This produces trajectories where intermediate results are more accurate and final answers are more reliable, reducing the noise in training data.

\paragraph{Scalable interaction depth.}
The multi-agent structure naturally scales the depth of interaction without increasing the burden on any single agent's context window.
Complex questions that require extensive exploration can be handled by distributing the search across focused sub-tasks, each with manageable context requirements.

\paragraph{Rich behavioral patterns.}
By generating training data through multi-agent collaboration, the model learns behavioral patterns---task decomposition, intermediate verification, and error-driven re-exploration---that improve its general reasoning ability, benefiting both single-agent and multi-agent deployment scenarios.


==> sections/reinforcement_learning.tex <==
% =============================================================================
% Section 6: Reinforcement Learning
% =============================================================================

\section{Reinforcement Learning}
\label{sec:rl}

After supervised fine-tuning, we further improve the agent's capabilities through reinforcement learning (RL) with environmental interaction.
This stage enables the model to explore beyond the boundaries of demonstration data and develop its own strategies for complex research tasks through trial-and-error learning.

\subsection{Problem Formulation}
\label{sec:rl-formulation}

We formulate the deep research task as a sequential decision-making problem.
Given a question $q$, the agent produces an interaction trajectory $\mathcal{H} = \{(\tau_1, a_1, o_1), \ldots, (\tau_T, a_T, o_T)\}$, where $\tau_t$ denotes the agent's reasoning at step $t$, $a_t$ denotes the action (tool call or answer generation), and $o_t$ denotes the environment observation.
The policy $\pi_\theta$ generates each thought--action pair conditioned on the trajectory history:
\begin{equation}
\tau_t, a_t \sim \pi_\theta(\cdot \mid q, \mathcal{H}_{<t}).
\end{equation}

Upon trajectory completion, a reward $R(q, \mathcal{H})$ is computed based on the correctness of the final answer.
The training objective is to find parameters $\theta^*$ that maximize the expected reward across the training distribution.


\subsection{Reward Design}
\label{sec:rl-reward}

\textcolor{red}{[To be elaborated once RL reward design is finalized.]}

We design the reward signal based on answer correctness as the primary criterion.
For questions with verifiable ground-truth answers, the reward is determined by exact or fuzzy matching against the reference answer:
\begin{equation}
R(q, \mathcal{H}) = \begin{cases} 1, & \text{if } a_T \text{ matches the ground-truth answer} \\ 0, & \text{otherwise} \end{cases}
\end{equation}

\textcolor{red}{[Potential extensions to be described: (1) verifier-based reward signals for questions without exact ground truth, (2) intermediate step rewards, (3) reward shaping for trajectory quality.]}


\subsection{Training Algorithm}
\label{sec:rl-algorithm}

\textcolor{red}{[To be elaborated once the specific RL algorithm (e.g., GRPO, PPO) and training details are finalized.]}

We employ \textcolor{red}{[algorithm name]} as our RL training algorithm, which optimizes the policy through on-policy rollouts in a real web environment.
Key design considerations include:

\paragraph{Real-world environment interaction.}
During RL training, the agent interacts with real web search engines and websites, producing authentic observation signals.
This ensures that the learned policy is directly applicable to real deployment conditions, avoiding the sim-to-real gap that arises from simulated environments~\cite{Tongyi-DeepResearch}.
% cite: Tongyi DeepResearch (environment design discussion)

\paragraph{Sandbox environment optimization.}
\textcolor{red}{[To be described: sandbox setup for safe and efficient RL training, including containerization, timeout handling, and caching mechanisms.]}

\paragraph{Training acceleration.}
\textcolor{red}{[To be described: techniques for accelerating agentic RL training, including parallel rollout, caching of search results, and efficient trajectory processing.]}

\paragraph{Long-trajectory challenges.}
Deep research tasks often produce extremely long trajectories that pose challenges for RL training in terms of both credit assignment and computational cost.
\textcolor{red}{[To be described: specific solutions for handling long trajectories, e.g., length normalization~\cite{SFR-DeepResearch}, trajectory truncation strategies, or reward denoising mechanisms~\cite{AgentCPM-Explore}.]}
% cite: SFR-DeepResearch (length-normalized RL), AgentCPM-Explore (reward denoising)


==> sections/test_time_scaling.tex <==
% =============================================================================
% Section 7: Test-time Scaling and Inference Strategies
% =============================================================================

\section{Test-time Scaling and Inference Strategies}
\label{sec:test-time}

Beyond training-time improvements, we explore strategies for enhancing model performance at inference time.
We present two complementary approaches: context management for sustained long-horizon reasoning, and multi-agent inference as a novel test-time scaling paradigm.


\subsection{Context Management}
\label{sec:context-management}

Long-horizon research tasks generate extensive interaction histories that can quickly exhaust the model's context window, leading to degraded performance as critical earlier information is displaced by recent observations.
We employ context management strategies to maintain effective reasoning capacity across arbitrarily long research sessions.

\textcolor{red}{[To be elaborated once context management details are finalized. Key aspects to be described:]}

\paragraph{Dynamic context window management.}
\textcolor{red}{[Description of how the context window is dynamically managed during inference, including strategies for retaining the most informative past interactions while discarding redundant content.]}

\paragraph{Long-trajectory compression.}
\textcolor{red}{[Description of compression mechanisms for maintaining essential information from earlier interaction steps, potentially including structured state representations or summary-based approaches.]}

\paragraph{Memory management.}
\textcolor{red}{[Description of explicit memory mechanisms that allow the agent to store and retrieve key findings beyond the immediate context window.]}


\subsection{Multi-Agent Inference Strategy}
\label{sec:multi-agent-inference}

A distinctive feature of our approach is that the multi-agent training paradigm naturally enables multi-agent inference at test time.
We introduce multi-agent inference as a new dimension of test-time scaling, complementary to existing approaches based on extended reasoning chains, increased context windows, or best-of-N sampling.

\paragraph{Motivation.}
Existing test-time scaling methods primarily operate along a single axis: allocating more computation to a single model instance, whether through longer reasoning chains~\cite{MiroThinker}, extended context windows, or multiple independent sampling attempts.
% cite: MiroThinker (interactive scaling)
While effective, these approaches are fundamentally limited by the single agent's capacity to simultaneously manage planning, execution, and verification within one decision-making loop.
We observe that our multi-agent training data (Section~\ref{sec:multi-agent-framework}) encodes structured patterns of task decomposition, focused execution, and systematic verification.
If the model has effectively learned these patterns during training, it should be possible to leverage them at inference time by deploying the same multi-agent collaboration structure used during data synthesis.

\paragraph{Multi-agent inference architecture.}
At inference time, we deploy the trained model in a multi-agent configuration that mirrors the training data generation process:
\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item The \textbf{main-agent} receives the user's question and generates a high-level plan by decomposing it into focused sub-tasks. It coordinates the overall research process and synthesizes the final answer.
    \item The \textbf{search sub-agent(s)} receive individual sub-task queries from the main-agent and perform focused information retrieval. Multiple sub-agents can operate in parallel on different sub-tasks, improving efficiency.
    \item The \textbf{verifier agent} validates intermediate results and the final answer, triggering revision when verification fails.
\end{itemize}

The key insight is that a single backbone model can fulfill all three roles through appropriate prompting and context configuration, as the model has been trained on trajectories containing all three behavioral patterns.

\paragraph{Training-inference consistency.}
The effectiveness of multi-agent inference rests on the principle of training-inference consistency: the model performs best when the inference paradigm aligns with the paradigm under which training data was generated.
Since our training trajectories encode explicit patterns of task decomposition (main-agent behavior), focused retrieval (sub-agent behavior), and quality verification (verifier behavior), the model can leverage these internalized patterns most effectively when deployed in a matching multi-agent configuration.
This contrasts with single-agent inference, where the model must simultaneously exhibit all these behaviors within a single decision loop, potentially conflating or under-utilizing the specialized patterns learned during training.


\paragraph{Advantages.}
Multi-agent inference offers several benefits over single-agent deployment:
(1) \textit{Structured task decomposition}---the main-agent can focus entirely on strategic planning without being interrupted by search operations;
(2) \textit{Parallel execution}---multiple sub-agents can work on different sub-tasks simultaneously, improving throughput;
(3) \textit{Systematic quality control}---the verifier agent provides an independent check at each stage, preventing error propagation;
and (4) \textit{Context efficiency}---each agent maintains a focused context relevant to its role, avoiding context dilution that occurs when a single agent must track all aspects simultaneously.


\subsection{Other Test-time Scaling Methods}
\label{sec:other-test-time}

\textcolor{red}{[To be elaborated once additional test-time scaling strategies are finalized. Potential content includes:]}

\textcolor{red}{[Best-of-N sampling with verifier-based selection, where the verifier agent scores multiple candidate answers and selects the most reliable one.]}

\textcolor{red}{[Adaptive computation allocation, where the inference budget (number of tool calls, search depth) is dynamically adjusted based on question difficulty or the model's confidence level.]}


==> sections/trajectory_optimization.tex <==
% =============================================================================
% Section 5: Trajectory Optimization
% =============================================================================

\section{Trajectory Optimization}
\label{sec:trajectory-optimization}

Not all trajectories generated by the multi-agent framework succeed in reaching the correct answer.
Rather than discarding these erroneous trajectories, we argue that they contain valuable learning signals: failed trajectories reveal common failure modes, identify challenging sub-problems, and provide natural starting points for injecting self-reflection behaviors.
In this section, we introduce two complementary trajectory optimization strategies that transform erroneous trajectories into effective training resources.

\subsection{Motivation}
\label{sec:traj-opt-motivation}

Erroneous trajectories are a natural byproduct of any data synthesis pipeline, and their prevalence increases with question difficulty.
We observe that these trajectories, while incorrect in their final answers, often contain partially correct reasoning chains, useful intermediate findings, and informative failure points.
Discarding them entirely wastes a substantial fraction of synthesis effort and, more importantly, forfeits the opportunity to teach the model \textit{how to recover from mistakes}---a capability that is critical for robust research agents.

Our trajectory optimization strategy explicitly injects self-reflection patterns into the training data, teaching the model to recognize its own errors and revise its approach.
This strategy leverages the verifier agent (Section~\ref{sec:framework-arch}) to identify which trajectories require optimization and to guide the recovery process.


\subsection{Reflection-Guided Re-rollout}
\label{sec:traj-reflection}

We explicitly inject self-reflection patterns into the model's behavioral repertoire through reflection-guided re-rollout.

\paragraph{Core idea.}
Given an erroneous trajectory $\mathcal{T}^-$ for question $q$, we construct a \textit{reflection-augmented trajectory} that demonstrates the process of recognizing an error, reflecting on its cause, and successfully revising the approach.
This provides the model with explicit training examples of the self-correction behavior that is largely absent from standard trajectory data.

\paragraph{Reflection and re-rollout process.}
The process operates in three steps:
\begin{enumerate}[leftmargin=*, itemsep=2pt]
    \item \textbf{Error identification:} The verifier agent analyzes the erroneous trajectory $\mathcal{T}^-$ and identifies the specific point(s) of failure, producing a structured error analysis that pinpoints incorrect reasoning steps or faulty information retrieval.
    \item \textbf{Reflection generation:} Based on the error analysis, a reflection segment is generated that explicitly articulates: (a) what went wrong in the original approach, (b) why the error occurred, and (c) what alternative strategy should be adopted. This reflection is appended to the trajectory context.
    \item \textbf{Re-rollout:} Starting from the reflection, the agent re-executes the research process with the revised strategy, producing a new trajectory segment. If the re-rollout reaches the correct answer, the complete sequence---original attempt, error identification, reflection, and successful revision---forms a reflection-augmented training example.
\end{enumerate}

\paragraph{Training with reflection data.}
The reflection-augmented trajectories are incorporated into the SFT training set, providing the model with explicit demonstrations of the think--reflect--revise cycle.
This approach directly injects the self-reflection behavioral pattern that we identified as lacking in existing trajectory data (Section~\ref{sec:introduction}).

The reflection-augmented trajectories equip the model with the practical skill of self-correction---recognizing errors and revising strategies---a capability that is largely absent from standard trajectory data. The effectiveness of this approach is validated by our analysis experiments in Section~\ref{sec:experiments}.

